Computational Benefits of Intermediate Rewards for Goal-Reaching Policy Learning

Many goal-reaching reinforcement learning (RL) tasks have empirically verified that rewarding the agent on subgoals improves convergence speed and practical performance. We attempt to provide a theoretical framework to quantify the computational benefits of rewarding the completion of subgoals, in terms of the number of synchronous value iterations. In particular, we consider subgoals as one-way {\em intermediate states}, which can only be visited once per episode and propose two settings that consider these one-way intermediate states: the one-way single-path (OWSP) and the one-way multi-path (OWMP) settings. In both OWSP and OWMP settings, we demonstrate that adding {\em intermediate rewards} to subgoals is more computationally efficient than only rewarding the agent once it completes the goal of reaching a terminal state. We also reveal a trade-off between computational complexity and the pursuit of the shortest path in the OWMP setting: adding intermediate rewards significantly reduces the computational complexity of reaching the goal but the agent may not find the shortest path, whereas with sparse terminal rewards, the agent finds the shortest path at a significantly higher computational cost. We also corroborate our theoretical results with extensive experiments on the MiniGrid environments using Q-learning and some popular deep RL algorithms.

==> Total_States.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{lcccc}
        \toprule
        \multicolumn{1}{c}{} & \multicolumn{1}{c}{Dots} & \multicolumn{1}{c}{Pacman} &\multicolumn{1}{c}{Ghost}& \multicolumn{1}{c}{\# of States}\\
        \midrule
        Case 1 & Mid \& Bot & 7 & 9 & 63\\
        Case 2 & Mid & 8 & 9 & 72 \\
        Case 3 & Bot & 8 & 9 & 72\\
        Case 4 & None & 2 & 9 & 18\\
        
        Total  &  &  &  & 225\\
        \bottomrule
    \end{tabular}
    \caption{Calculation of the total states. Each state consists different status of dots, position of the Pacman, and the position of the ghost.}
    \label{tab:Total_States}
\end{table}



==> maze/maze.tex <==
\begin{tikzpicture}[scale=0.5]
\centering
\draw[step=1cm, gray, very thin] (0, -13) grid (13, 0);
% upper boundary
\fill[black] (0, 0) rectangle (1, -1);
\fill[black] (1, 0) rectangle (2, -1);
\fill[black] (2, 0) rectangle (3, -1);
\fill[black] (3, 0) rectangle (4, -1);
\fill[black] (4, 0) rectangle (5, -1);
\fill[black] (5, 0) rectangle (6, -1);
\fill[black] (6, 0) rectangle (7, -1);
\fill[black] (7, 0) rectangle (8, -1);
\fill[black] (8, 0) rectangle (9, -1);
\fill[black] (9, 0) rectangle (10, -1);
\fill[black] (10, 0) rectangle (11, -1);
\fill[black] (11, 0) rectangle (12, -1);
\fill[black] (12, 0) rectangle (13, -1);
% left boundary, left one blank for starting point

\fill[black] (0, -2) rectangle (1, -3);
\fill[black] (0, -3) rectangle (1, -4);
\fill[black] (0, -4) rectangle (1, -5);
\fill[black] (0, -5) rectangle (1, -6);
\fill[black] (0, -6) rectangle (1, -7);
\fill[black] (0, -7) rectangle (1, -8);
\fill[black] (0, -8) rectangle (1, -9);
\fill[black] (0, -9) rectangle (1, -10);
\fill[black] (0, -10) rectangle (1, -11);
\fill[black] (0, -11) rectangle (1, -12);
\fill[black] (0, -12) rectangle (1, -13);
% lower boundary
\fill[black] (1, -12) rectangle (2, -13);
\fill[black] (2, -12) rectangle (3, -13);
\fill[black] (3, -12) rectangle (4, -13);
\fill[black] (4, -12) rectangle (5, -13);
\fill[black] (5, -12) rectangle (6, -13);
\fill[black] (6, -12) rectangle (7, -13);
\fill[black] (7, -12) rectangle (8, -13);
\fill[black] (8, -12) rectangle (9, -13);
\fill[black] (9, -12) rectangle (10, -13);
\fill[black] (10, -12) rectangle (11, -13);
\fill[black] (11, -12) rectangle (12, -13);
\fill[black] (12, -12) rectangle (13, -13);
% right boundary, left one blank for the exist
\fill[black] (12, -1) rectangle (13, -2);
\fill[black] (12, -2) rectangle (13, -3);
\fill[black] (12, -3) rectangle (13, -4);
\fill[black] (12, -4) rectangle (13, -5);
\fill[black] (12, -5) rectangle (13, -6);
\fill[black] (12, -6) rectangle (13, -7);
\fill[black] (12, -7) rectangle (13, -8);
\fill[black] (12, -8) rectangle (13, -9);
\fill[black] (12, -9) rectangle (13, -10);
\fill[black] (12, -10) rectangle (13, -11);

% fill in content of the maze, row 3
\fill[black] (2, -2) rectangle (3, -3);
\fill[black] (3, -2) rectangle (4, -3);
\fill[black] (4, -2) rectangle (5, -3);
\fill[black] (5, -2) rectangle (6, -3);
\fill[black] (6, -2) rectangle (7, -3);
\fill[black] (7, -2) rectangle (8, -3);
\fill[black] (8, -2) rectangle (9, -3);
% \fill[black] (9, -2) rectangle (10, -3);
\fill[black] (10, -2) rectangle (11, -3);
% row 4
\fill[black] (2, -3) rectangle (3, -4);
\fill[black] (4, -3) rectangle (5, -4);
\fill[black] (8, -3) rectangle (9, -4);
\fill[black] (10, -3) rectangle (11, -4);
% row 5
\fill[black] (2, -4) rectangle (3, -5);
\fill[black] (4, -4) rectangle (5, -5);
\fill[black] (6, -4) rectangle (7, -5);
\fill[black] (8, -4) rectangle (9, -5);
\fill[black] (10, -4) rectangle (11, -5);
% row 6
\fill[black] (2, -5) rectangle (3, -6);
\fill[black] (4, -5) rectangle (5, -6);
\fill[black] (6, -5) rectangle (7, -6);
\fill[black] (8, -5) rectangle (9, -6);
\fill[black] (10, -5) rectangle (11, -6);
% row 7
\fill[black] (4, -6) rectangle (5, -7);
\fill[black] (6, -6) rectangle (7, -7);
\fill[black] (8, -6) rectangle (9, -7);
\fill[black] (9, -6) rectangle (10, -7);
\fill[black] (10, -6) rectangle (11, -7);
% row 7
\fill[black] (2, -7) rectangle (3, -8);
\fill[black] (4, -7) rectangle (5, -8);
\fill[black] (6, -7) rectangle (7, -8);
\fill[black] (8, -7) rectangle (9, -8);
% row 8
\fill[black] (2, -8) rectangle (3, -9);
\fill[black] (4, -8) rectangle (5, -9);
\fill[black] (6, -8) rectangle (7, -9);
\fill[black] (8, -8) rectangle (9, -9);
\fill[black] (10, -8) rectangle (11, -9);
\fill[black] (11, -8) rectangle (12, -9);
% row 9
\fill[black] (2, -9) rectangle (3, -10);
\fill[black] (6, -9) rectangle (7, -10);
\fill[black] (8, -9) rectangle (9, -10);
% row 10
\fill[black] (2, -10) rectangle (3, -11);
\fill[black] (3, -10) rectangle (4, -11);
\fill[black] (4, -10) rectangle (5, -11);
\fill[black] (5, -10) rectangle (6, -11);
\fill[black] (6, -10) rectangle (7, -11);
\fill[black] (8, -10) rectangle (9, -11);
\fill[black] (9, -10) rectangle (10, -11);
\fill[black] (10, -10) rectangle (11, -11);
\fill[black] (11, -10) rectangle (12, -11);
% row 12
\fill[black] (6, -11) rectangle (7, -12);

% draw start and end
\draw[->, thick](-1.0,-1.5) -- (-0.5,-1.5) node [pos=0,left,font=\footnotesize] {start};
\draw[->, thick](13.5,-11.5) -- (14.0,-11.5) node [pos=1,right,font=\footnotesize] {finish};

\fill[blue!50!white] (0.5, -1.5) circle (0.3cm);
\fill[green!50!white] (12.5, -11.5) circle (0.3cm);
\fill[cyan!50!white] (7.5, -3.5) circle (0.3 cm);
\draw[cyan, line width=3] (0.5, -1.5) -- (1.5, -1.5) -- (1.5, -6.5) -- (3.5, -6.5) -- (3.5, -9.5) -- (5.5, -9.5) -- (5.5, -3.5) -- (7.5, -3.5) -- (7.5, -11.5) -- (12.5, -11.5);

%% legend
% Bounding Box
\draw[black] (14,-1) -- (14,-5) -- (16.5,-5) -- (16.5,-1) -- (14,-1);
% Drawing
\fill[blue!50!white] (14.5, -1.5) circle (0.3cm);
\fill[green!50!white] (14.5, -2.5) circle (0.3cm);
\draw[cyan, line width=3] (14.2,-3.5) -- (14.8,-3.5);
\fill[cyan!50!white] (14.5, -4.5) circle (0.3cm);
% Caption
\node [right,font=\footnotesize] (a) at (15,-1.5) {$s_0$};
\node [right,font=\footnotesize] (b) at (15,-2.5) {$\mc S_{T}$};
\node [right,font=\footnotesize] (c) at (15,-3.5) {$\mc S_I$};
\node [right,font=\footnotesize] (d) at (15,-4.5) {$s_i$};
\end{tikzpicture}

==> maze/maze_c.tex <==
\begin{tikzpicture}[scale=0.6]
\centering
\draw[step=1cm, gray, very thin] (0, -13) grid (13, 0);
% upper boundary
\fill[black] (0, 0) rectangle (1, -1);
\fill[black] (1, 0) rectangle (2, -1);
\fill[black] (2, 0) rectangle (3, -1);
\fill[black] (3, 0) rectangle (4, -1);
\fill[black] (4, 0) rectangle (5, -1);
\fill[black] (5, 0) rectangle (6, -1);
\fill[black] (6, 0) rectangle (7, -1);
\fill[black] (7, 0) rectangle (8, -1);
\fill[black] (8, 0) rectangle (9, -1);
\fill[black] (9, 0) rectangle (10, -1);
\fill[black] (10, 0) rectangle (11, -1);
% \fill[black] (11, 0) rectangle (12, -1);
\fill[black] (12, 0) rectangle (13, -1);
% left boundary, left one blank for starting point

\fill[black] (0, -2) rectangle (1, -3);
\fill[black] (0, -3) rectangle (1, -4);
\fill[black] (0, -4) rectangle (1, -5);
\fill[black] (0, -5) rectangle (1, -6);
\fill[black] (0, -6) rectangle (1, -7);
\fill[black] (0, -7) rectangle (1, -8);
\fill[black] (0, -8) rectangle (1, -9);
\fill[black] (0, -9) rectangle (1, -10);
\fill[black] (0, -10) rectangle (1, -11);
\fill[black] (0, -11) rectangle (1, -12);
\fill[black] (0, -12) rectangle (1, -13);
% lower boundary
% \fill[black] (1, -12) rectangle (2, -13);
\fill[black] (2, -12) rectangle (3, -13);
\fill[black] (3, -12) rectangle (4, -13);
\fill[black] (4, -12) rectangle (5, -13);
\fill[black] (5, -12) rectangle (6, -13);
\fill[black] (6, -12) rectangle (7, -13);
\fill[black] (7, -12) rectangle (8, -13);
\fill[black] (8, -12) rectangle (9, -13);
\fill[black] (9, -12) rectangle (10, -13);
\fill[black] (10, -12) rectangle (11, -13);
\fill[black] (11, -12) rectangle (12, -13);
\fill[black] (12, -12) rectangle (13, -13);
% right boundary, left one blank for the exist
\fill[black] (12, -1) rectangle (13, -2);
\fill[black] (12, -2) rectangle (13, -3);
\fill[black] (12, -3) rectangle (13, -4);
\fill[black] (12, -4) rectangle (13, -5);
\fill[black] (12, -5) rectangle (13, -6);
\fill[black] (12, -6) rectangle (13, -7);
\fill[black] (12, -7) rectangle (13, -8);
\fill[black] (12, -8) rectangle (13, -9);
\fill[black] (12, -9) rectangle (13, -10);
\fill[black] (12, -10) rectangle (13, -11);

% fill in content of the maze, row 3
\fill[black] (2, -2) rectangle (3, -3);
\fill[black] (3, -2) rectangle (4, -3);
\fill[black] (4, -2) rectangle (5, -3);
\fill[black] (5, -2) rectangle (6, -3);
\fill[black] (6, -2) rectangle (7, -3);
\fill[black] (7, -2) rectangle (8, -3);
\fill[black] (8, -2) rectangle (9, -3);
% \fill[black] (9, -2) rectangle (10, -3);
\fill[black] (10, -2) rectangle (11, -3);
% row 4
\fill[black] (2, -3) rectangle (3, -4);
\fill[black] (4, -3) rectangle (5, -4);
\fill[black] (8, -3) rectangle (9, -4);
\fill[black] (10, -3) rectangle (11, -4);
% row 5
\fill[black] (2, -4) rectangle (3, -5);
\fill[black] (4, -4) rectangle (5, -5);
\fill[black] (6, -4) rectangle (7, -5);
\fill[black] (8, -4) rectangle (9, -5);
\fill[black] (10, -4) rectangle (11, -5);
% row 6
\fill[black] (2, -5) rectangle (3, -6);
\fill[black] (4, -5) rectangle (5, -6);
\fill[black] (6, -5) rectangle (7, -6);
\fill[black] (8, -5) rectangle (9, -6);
\fill[black] (10, -5) rectangle (11, -6);
% row 7
\fill[black] (4, -6) rectangle (5, -7);
\fill[black] (6, -6) rectangle (7, -7);
\fill[black] (8, -6) rectangle (9, -7);
\fill[black] (9, -6) rectangle (10, -7);
\fill[black] (10, -6) rectangle (11, -7);
% row 7
\fill[black] (2, -7) rectangle (3, -8);
\fill[black] (4, -7) rectangle (5, -8);
\fill[black] (6, -7) rectangle (7, -8);
\fill[black] (8, -7) rectangle (9, -8);
% row 8
\fill[black] (2, -8) rectangle (3, -9);
\fill[black] (4, -8) rectangle (5, -9);
\fill[black] (6, -8) rectangle (7, -9);
\fill[black] (8, -8) rectangle (9, -9);
\fill[black] (10, -8) rectangle (11, -9);
\fill[black] (11, -8) rectangle (12, -9);
% row 9
\fill[black] (2, -9) rectangle (3, -10);
\fill[black] (6, -9) rectangle (7, -10);
\fill[black] (8, -9) rectangle (9, -10);
% row 10
\fill[black] (2, -10) rectangle (3, -11);
\fill[black] (3, -10) rectangle (4, -11);
\fill[black] (4, -10) rectangle (5, -11);
\fill[black] (5, -10) rectangle (6, -11);
\fill[black] (6, -10) rectangle (7, -11);
\fill[black] (8, -10) rectangle (9, -11);
\fill[black] (9, -10) rectangle (10, -11);
% \fill[black] (10, -10) rectangle (11, -11);
\fill[black] (11, -10) rectangle (12, -11);
% row 12
% \fill[black] (6, -11) rectangle (7, -12);

% draw start and end
\draw[->, thick](-1.0,-1.5) -- (-0.5,-1.5) node [pos=0,left,font=\footnotesize] {start};
\draw[->, thick](13.5,-11.5) -- (14.0,-11.5) node [pos=1,right,font=\footnotesize] {good ending};
\draw[->, thick](1.5,-13.5) -- (1.5,-14.0) node [pos=1.0,below,font=\footnotesize] {bad ending};
\draw[->, thick](11.5,0.5) -- (11.5,1.0) node [pos=1.0,above,font=\footnotesize] {bad ending};

\fill[blue!50!white] (0.5, -1.5) circle (0.4cm);
\fill[red!50!white] (1.5, -12.5) circle (0.4cm);
\fill[red!50!white] (11.5, -0.5) circle (0.4cm);
\fill[green!50!white] (12.5, -11.5) circle (0.4cm);
% Necessary states
\draw[cyan, line width=3] (0.5, -1.5) -- (1.5,-1.5);
\draw[cyan, line width=3] (10.5, -11.5) -- (12.5,-11.5);
% Intermediate states
\draw[blue, dashed, thick] (1.5, -6.5) -- (3.5, -6.5) -- (3.5, -9.5) -- (5.5, -9.5) -- (5.5, -3.5) -- (7.5, -3.5) -- (7.5, -11.5);
\draw[blue, dashed, thick] (1.5, -1.5) -- (11.5, -1.5) -- (11.5,-7.5) -- (9.5 , -7.5) -- (9.5, -9.5) -- (10.5, -9.5) -- (10.5, -11.5);
\draw[purple, dashed, thick] (1.5, -1.5) -- (1.5, -11.5) -- (10.5, -11.5);

% legend
\draw[black] (14,-1) -- (14,-6) -- (16.5,-6) -- (16.5,-1) -- (14,-1);
\fill[blue!50!white] (14.5, -1.5) circle (0.3cm);
\fill[green!50!white] (14.5, -2.5) circle (0.3cm);
\fill[red!50!white] (14.5, -3.5) circle (0.3cm);
\draw[cyan, line width=3] (14.2,-4.5) -- (14.8,-4.5);
\draw[purple, dashed, thick] (14.2,-5.6) -- (14.8,-5.6);
\draw[blue, dashed, thick] (14.2,-5.4) -- (14.8,-5.4);

\node [right,font=\footnotesize] (a) at (15,-1.5) {$\mc S_S$};
\node [right,font=\footnotesize] (b) at (15,-2.5) {$\mc S_{T^+}$};
\node [right,font=\footnotesize] (c) at (15,-3.5) {$\mc S_{T^-}$};
\node [right,font=\footnotesize] (d) at (15,-4.5) {$\mc S_N$};
\node [right,font=\footnotesize] (e) at (15,-5.5) {$\mc S_I$};
\end{tikzpicture}

==> mdp_graph/setting2.tex <==
\begin{tikzpicture}[scale=0.75]
\centering
% draw start and end
% s0 -> sj1
\draw[fill=white] (0.5, 0.5) circle (0.3cm);
\node [below,font=\footnotesize] at (0.5,0) {$s_0$};
\draw[black] (1, 0.6) -- (1.8, 2.5);
\draw[black] (1, 0.4) -- (1.8, -1.5);
\node [font=\footnotesize] at (2.5,2.5) {$\dots$};
\node [font=\footnotesize] at (2.5,0.75) {$\vdots$};
\node [font=\footnotesize] at (2.5,-1.5) {$\dots$};
\draw[->,black] (3.2, 2.5) -- (4, 2.5);
\draw[->,black] (3.2, -1.5) -- (4, -1.5);
\draw[fill=white] (4.5, 2.5) circle (0.3cm);
\node [below,font=\footnotesize] at (4.5,2.0) {$s_{i_{j_1}}$};
\draw[fill=white] (4.5, -1.5) circle (0.3cm);
\node [below,font=\footnotesize] at (4.5,-2.0) {$s_{i_{j^\prime_1}}$};

% -> sj2
\draw[black] (5, 2.6) -- (5.8, 3.5);
\draw[black] (5, 2.4) -- (5.8, 1.5);
\node [font=\footnotesize] at (6.5,3.5) {$\dots$};
\node [font=\footnotesize] at (6.5,2.75) {$\vdots$};
\node [font=\footnotesize] at (6.5,1.5) {$\dots$};
\draw[->,black] (7.2, 3.5) -- (8, 2.6);
\draw[->,black] (7.2, 1.5) -- (8, 2.4);

\draw[fill=white] (8.5, 2.5) circle (0.3cm);
\node [below,font=\footnotesize] at (8.5,2) {$s_{i_{j_2}}$};

\draw[black] (5, -1.4) -- (5.8, -0.5);
\draw[black] (5, -1.6) -- (5.8, -2.5);
\node [font=\footnotesize] at (6.5,-0.5) {$\dots$};
\node [font=\footnotesize] at (6.5,-1.25) {$\vdots$};
\node [font=\footnotesize] at (6.5,-2.5) {$\dots$};
\draw[->,black] (7.2, -0.5) -- (8, -1.4);
\draw[->,black] (7.2, -2.5) -- (8, -1.6);

\draw[fill=white] (8.5, -1.5) circle (0.3cm);
\node [below,font=\footnotesize] at (8.5,-2) {$s_{i_{j^\prime_2}}$};

% -> ... -> sn
\draw[black] (9, 2.5) -- (9.8, 2.5);
\draw[->,black] (11.2, 2.5) -- (12, 2.5);
\node [font=\footnotesize] at (10.5,2.5) {$\dots$};
\draw[fill=white] (12.5, 2.5) circle (0.3cm);
\node [below,font=\footnotesize] at (12.5,2.0) {$s_{i_{j_m}}$};

\node [font=\footnotesize] at (10.5,0.75) {$\vdots$};

\draw[black] (9, -1.5) -- (9.8, -1.5);
\draw[->,black] (11.2, -1.5) -- (12, -1.5);
\node [font=\footnotesize] at (10.5,-1.5) {$\dots$};
\draw[fill=white] (12.5, -1.5) circle (0.3cm);
\node [below,font=\footnotesize] at (12.5,-2.0) {$s_{i_{j^\prime_{m^\prime}}}$};


% -> sT+
\draw[black] (13.0, 2.5) -- (13.8, 2.5);
\node [font=\footnotesize] at (14.5,2.5) {$\dots$};
\node [font=\footnotesize] at (14.5,0.75) {$\vdots$};
\draw[black] (13.0, -1.5) -- (13.8, -1.5);
\node [font=\footnotesize] at (14.5,-1.5) {$\dots$};
\node [below,font=\footnotesize] at (16.5,0) {$\mc S_{T}$};
\draw[->,black] (15.2, 2.5) -- (16.0, 0.6);
\draw[->,black] (15.2, -1.5) -- (16.0, 0.4);
\draw[fill=white] (16.5, 0.5) circle (0.3cm);
\draw[fill=white] (16.5, 0.5) circle (0.2cm);

\end{tikzpicture}

==> misc.tex <==
\subsection{Motivation}
We study the sparse Model-Based RL simply because the state transition matrix of many real world applications are very sparse. That is, many applications, only a few actions in the action set are valid, moreover, given a state $s$ and all of its valid actions $a$, the possible outcome states $s^\prime$ are very limited in the state space.

\paragraph{Sparse model.}
By the nature of many tabular MDP problems, we assume that the state transition matrix $\mb P, \mb P_\pi,\mb P^\pi$ are ``extremely'' sparse, and the state-action pairs $(s,a)$ is ``relatively'' sparse. 

\paragraph{The Pacman example.}

In the following Pacman problem shown in Figure \ref{fig:Pacman}, when there are only two fixed dots in the maze and one ghost, there are 225 different states in total ($|\mc S|=225$, see detailed calculation in Table \ref{tab:Total_States}). The action set contains 4 different elements $\mc A = \{\text{up},\text{down},\text{left},\text{right}\}$. Let the following matrix 
\begin{equation*}
    \begin{bmatrix}
        1&2&3\\
        4&5&6\\
        7&8&9
    \end{bmatrix}
\end{equation*} 
denote the position index of the Pacman game in Figure \ref{fig:Pacman}, the Pacman game naturally satisfies the sparsity assumption (\cite{dubeyICLRW18human,yang2020harnessing} the first paper observes a sparse visited state, and the second paper shows that the state-action pair ($Q$ function) has low-rank structure):
\begin{itemize}
    \item \textbf{``Relativly'' sparse state-action pairs}: at location 5, the pacman only has one valid action (right), at location 6, the Pacman has three valid actions (up, down, left), at the other locations, the pacman only has 2 valid actions. Hence, the valid state-action matrix are 50\% sparse.
    \item \textbf{``Extremely'' sparse probability transition vector}: The probability transition vectors $P(s^\prime|s,a)\in \bb R^{225}$ is extremely sparse, because the ghost also has at most three actions after the Pacman moves and the maximum is achieved when the ghost is at location 6. Therefore, the vector $P(s^\prime|s,a)\in \bb R^{225}$ is a 3-sparse (most of the time a 2-sparse vector).
\end{itemize}


\input{Total_States}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0cm 0cm 0.1cm 0cm},clip]{fig/Pacman.png}
    \end{subfigure}
    \caption{The Pacman Game}
    \label{fig:Pacman}
\end{figure}
\subsection{Theoretical Results of Previous Works}
\begin{theorem}[Model-based planning \cite{agarwal2020model}] 
\label{thm:model-based-planning}
Suppose $\delta >0$ and $\eps \in \left(0,\frac{1}{\sqrt{1-\gamma}}\right]$. Let $\wh{\pi}$ be any $\eps_{opt}$-optimal policy for $\wh{M}$, i.e., $\norm{\wh{Q}^{\wh{\pi}}-\wh{Q}^\star}{\infty}\leq \eps_{opt}$. If 
\begin{equation*}
    N\geq \frac{c\gamma \log\left(c|\mc S||\mc A|(1-\gamma)^{-1}\delta^{-1}\right)}{(1-\gamma)^3\eps^2},
\end{equation*}
we have 
\begin{equation*}
    Q^{\wh{\pi}}(s,a)\geq Q^\star(s,a) -\eps - \frac{9\eps_{opt}}{1-\gamma} \quad \text{and} \quad V^{\wh{\pi}}(s)\geq V^\star(s) -\eps - \frac{9\eps_{opt}}{1-\gamma},\quad \forall (s,a) \in \mc S \times \mc A,
\end{equation*}
\end{theorem}
with probability at least $1-\delta$, where $c$ is an absolute constant, provided $\gamma \geq 1/2$.

\begin{theorem}[Perturbed model-based planning \cite{li2020breaking}]
\label{thm:perturb-model-based-planning}
There exists some universal constants $c_0,c_1>0$, such that: for any $\delta>0$ and any $\eps \in \left(0,\frac{1}{1-\gamma}\right]$, the policy $\wh{\pi}^\star_p$ obeys 
\begin{equation*}
    V^{\wh{\pi}^\star_p}(s)\geq V^\star(s)-\eps\quad \text{and} \quad Q^{\wh{\pi}^\star_p}(s,a)\geq Q^\star(s,a)-\gamma\eps,\quad \forall (s,a)\in \mc S\times \mc A
\end{equation*}
with probability at least $1-\delta$, provided that the perturbation size $\xi = \frac{c_1(1-\gamma)\eps}{|\mc S|^5|\mc A|^5}$ and the sample size per state-action pair exceeds 
\begin{equation}
    \label{eq:perturbed-sample-complexity}
    N\geq \frac{c_0\log\left(\frac{|\mc S||\mc A|}{(1-\gamma)\eps\delta}\right)}{(1-\gamma)^3\eps^2}.
\end{equation}
\end{theorem}
Note that $\wh{\pi}^\star_p$ is defined as 
\begin{equation}
    \wh \pi^\star_p:=\arg\max_{\pi} \wh V_p^\pi,
\end{equation}
and $\wh V^\pi_p$ is the value function of the perturbed empirical MDP $\wh M_p = (\mc S,\mc A,\wh P, r_p, \gamma)$ with probability transition kernel $\wh P$, where $r_p(s,a)$ is the {\em perturbed} reward
\begin{equation}
    r_p(s,a):=r(s,a)+\zeta(s,a),\quad \zeta(s,a)\overset{i.i.d.}{\sim}\msf{Unif}(0,\xi).
\end{equation}

\begin{remark}[Sample Complexity]
Table \ref{tab:previous_work} shows sample size range and sample complexity of previous works. Note that both Theorem \ref{thm:model-based-planning} and \ref{thm:perturb-model-based-planning} prove sample complexity for bounding {\em one} state-action pair $(s,a)\in\mc S\times \mc A$ and the overall sample complexity for the MDP problem is $|\mc S||\mc A|$ times the sample complexity of one state-action pair.
\end{remark}
\begin{remark}[Sample Complexity and Runtime]
Theorem \ref{thm:model-based-planning} and \ref{thm:perturb-model-based-planning} only provides the sample complexity of achieving an $\eps$-optimal policy, rather than providing an algorithm to solve the empirical MDP problem $\wh M$. In contrast, \cite{sidford2018near,sidford2018variance} provide algorithms (with runtime analysis) that solve the empirical MDP $\wh M$.
\end{remark}

\input{table/pre_work}

\subsection{Sparse Model-based Reinforcement Learning}
There are some immediate result we can get with the sparsity assumption.

\begin{itemize}
    \item  If we assume the state-action pair $(s,a)\in \mc S\times \mc A$ is $\theta$ sparse for some $\theta\in (0,1)$, that is, only $\theta|\mc S||\mc A|$ state-action pairs $(s,a)\in \mc S\times \mc A$ are valid. Suppose $N(\eps)$ is the minimum sample complexity for achieving an $\eps$-optimal policy, i.e., in \eqref{eq:perturbed-sample-complexity},
    \begin{equation*}
        N(\eps) = \frac{c_0|\mc S||\mc A|\log\left(\frac{|\mc S||\mc A|}{(1-\gamma)\eps\delta}\right)}{(1-\gamma)^3\eps^2}.   
    \end{equation*}
    Then the optimal sample complexity {\em at least} can be immediately reduced to $\theta N(\eps)$. In the Pacman case, we can {\em at least} reduce the sample complexity by half. 
    \item We can also assume the state transition kernel $P(s^\prime|s,a)$ is $\eta$ sparse, and $\eta\ll\theta$.
\end{itemize}
\paragraph{Potential contribution} We can try to exploit the sparsity assumption of state-action pair $(s,a)$ and the probability transition kernel $P(s^\prime|s,a)$ to obtain a sample complexity better than $\theta N(\eps)$ or an efficient {\em provable} algorithm. We may refer to \cite{agarwal2020model,li2020breaking} for the sample complexity and \cite{sidford2018near,sidford2018variance} for algorithms.

%%%%%%%
\sz{this paragraph is important when writing the introduction, especially when mentioning the practical evidence of intermediate rewards, leaving it here for reference, will include this paragraph into the introduction later.}
%%%%%%%
\paragraph{Relationship with Sparse Rewards and Dense Rewards.} Many practical RL works \cite{pathak2017curiosity,liu2018competitive} have suggested that RL algorithms generally perform better when dense rewards $r(s_a,s,a)$ are provided, but in reality, the nature of many tasks only provide sparse rewards at the terminal states \cite{levine2018learning,pathak2017curiosity,popov2017data,levine2018learning,silver2016mastering,silver2017mastering,tian2019elf}.\footnote{Also see \cite{li2017deep} for a survey.} As an MDP with only terminal rewards can be considered as the sparsest rewards setting of practical RL, designing intermediate rewards with prior knowledge on the intermediate states densifies the rewards hence improving the performance to at large.

\begin{proof}
\label{proof:absorb_radius_Q_learning}
\sz{will rewrite the whole proof later}
We will first introduce some notations. $\forall d\in \bb N^+$, we let $\mc S^{d}$ denote the set of states that is distance $d$ to the terminal state $s_{T^+}$:
\begin{equation*}
    \mc S^{(d)} = \{s\in\mc S|D(s,s_{T^+})=d\}.
\end{equation*}
Let $d$ be a positive integer such that $d\leq k$, $\forall s^d\in \mc S^{(d)}$ let $a^{d+}\in \mc A^+(s^d)$ denote a correction action of $s^d$ and $a^{d-}\notin\mc A^+(s^d)$ denote an incorrect action of $s^d$, we will use induction to prove the following claims $\forall k\in \bb N^+$:
\begin{equation}
    \label{eq:Induction_Claim}
    \begin{split}
        \text{Claim 1: }&Q_{k+1}(s^d,a^{d+})> Q_{k}(s^d,a^{d+}),\;\forall d\in\bb N^+, d\leq k\\ 
        \text{Claim 2: }&Q_{k}(s^{d^\prime},a^{d^\prime+})>Q_{k}(s^d,a^{d+}),\;\forall d^\prime \in \bb N^+, d^\prime<d\leq k,\\
        \text{Claim 3: }&Q_{k}(s^d,a^{d+})> Q_{k}(s^d,a^{d-}),\;\forall d\in\bb N^+, d\leq k
    \end{split}
\end{equation}
where the third claim directly imply that $s_{T+}$ in $\mc M$ with Q function $Q_k(\cdot,\cdot)$ has the absorbing radius $k$. Recall the expected Q learning update \eqref{eq:ExpQLearning}:
\begin{equation*}
    Q_{k+1}(s,a)\doteq(1-\alpha)Q_{k}(s,a)+\alpha\underset{s_a\sim P(\cdot|s,a)}{\bb E}\left(r(s,a,s_a)+\gamma \max_{a^\prime}Q_k(s_a,a^\prime)\right),\;\forall (s,a)\in \mc S\times \mc A.
\end{equation*}
We first check the above claims \eqref{eq:Induction_Claim} for the initial case $k=1,2$. We need include $k=2$ in the initial case, otherwise we cannot find a positive integer $d^\prime$ for Claim 2. We shall also note that $Q_k(s_{T^+},a) = 0,\forall a\in \mc A$, because the episode stops once the agent reaches the terminal state $s_{T^+}$ and hence $Q_k(s_{T^+},a)$ remains zero. 

\paragraph{Initial condition for $k=1$.}
We first check Claim 1 and Claim 3 for $k=1$. Since we only receive reward $r(s,a,s_a) = B$ when $s_a = s_{T^+}$, by the Q learning update, we have:
\begin{equation}
    Q_{1}(s,a) = 
    \begin{cases}
        \alpha(1-\eps)B, & \forall (s,a)\; \st\;s\in \mc S^1,a\in \mc A^+(s^1);\\
        0, &\text{otherwise,}
    \end{cases}
\end{equation}
and
\begin{equation}
    Q_{2}(s,a) = 
    \begin{cases}
        \alpha^2(1-\eps)^2\gamma B, & \forall (s,a)\; \st\;s\in \mc S^2,a\in \mc A^+(s^2);\\
        \alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X, & \forall (s,a)\; \st\;s\in \mc S^1,a\in \mc A^+(s^1);\\
        \alpha\gamma Y,&\forall (s,a)\; \st\;s\in \mc S^1,a\notin \mc A^+(s^1)\\
        0, &\text{otherwise,}
    \end{cases}
\end{equation}
where $X=\max_{a^\prime}Q_1(s_{a^{1+}},a^\prime)$ is largest Q value at the subsequent state $s_{a^{1+}}$, when a correct action is taken at $s^1$, but the agent fails to move forward to $s_{T^+}$ due to the randomness of the state action transition matrix $\mb P$ and $Y=\max_{a^\prime}Q_1(s_{a^{1-}},a^\prime)$ is the largest Q value at state $s_{a^{1-}}$, when an incorrect action $a^{1-}$ is taken at state $s^1$. 
By Assumption \ref{assump:min_step_correct_step}, we know that the $D(s_a,s_{T^+})\geq D(s,s_{T^+})=1$, hence we have: 
\begin{equation}
    0\leq X \leq \max_a(s^1,a) = Q_1(s^1,a^{1+})= \alpha(1-\eps)B.   
\end{equation}
Now we check Claim 1 and Claim 3 for $k=1$.\\
{\bf Claim 1:} $Q_{k+1}(s^d,a^{d+})> Q_{k}(s^d,a^{d+}),\;\forall d\in\bb N^+, d\leq k$.
\begin{equation}
        Q_2(s^1,a^{1+})= \alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X > \alpha(1-\eps) B = Q_1(s^1,a^{1+}),
\end{equation}
hence, Claim 1 is verified.\\
{\bf Claim 3:} $Q_{k}(s^d,a^{d+})> Q_{k}(s^d,a^{d-}),\; \forall d\in\bb N^+, d\leq k$.
\begin{equation}
    Q_1(s^1,a^{1+}) = \alpha(1-\eps) B >0 = Q_1(s^1,a^{1-}),
\end{equation}
hence, Claim 3 is verified.

\paragraph{Initial condition for $k=2$.}
We further compute one more step of the Q-learning to obtain $Q_3(s^1,a^{1+})$ and $Q_3(s^2,a^{2+})$.
\begin{equation}
    \label{eq:Q31Calculate}
    \begin{split}
        Q_3(s^1,a^{1+}) =& (1-\alpha)Q_2(s^1,a^{1+}) + \alpha\underset{s_a\sim P(\cdot|s^1,a^{1+})}{\bb E}\left(r(s^1,a^{1+},s_a)+\gamma \max_{a^\prime}Q_2(s_a,a^\prime)\right)\\
        =&(1-\alpha)\left[\alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X\right]+\alpha(1-\eps)B+\alpha\gamma\eps X^\prime\\
        =&\alpha(1-\alpha)^2(1-\eps)B+\alpha(1-\alpha)(1-\eps)B+\alpha(1-\alpha)\gamma\eps X+\alpha(1-\eps)B+\alpha\gamma \eps X^\prime\\
        =&\underbrace{\alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X}_{Q_2(s^1,a^{1+})}+\alpha(1-\alpha)^2(1-\eps)B-\alpha^2\gamma\eps X+\alpha\gamma\eps X^\prime,
    \end{split}
\end{equation}
and 
\begin{equation}
    \label{eq:Q32Calculate}
    \begin{split}
        &Q_3(s^2,a^{2+})\\
        =& (1-\alpha)Q_2(s^2,a^{2+}) + \alpha\underset{s_a\sim P(\cdot|s^2,a^{2+})}{\bb E}\left(r(s^2,a^{2+},s_a)+\gamma \max_{a^\prime}Q_2(s_a,a^\prime)\right)\\
        =&\alpha^2(1-\alpha)(1-\eps)^2\gamma B+\alpha\gamma(1-\eps)\left[\alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X\right]+\alpha\gamma\eps X^{\prime\prime}\\
        =& \alpha^2(1-\alpha)(1-\eps)^2\gamma B+\alpha^2(1-\alpha)(1-\eps)^2\gamma B+\underbrace{\alpha^2(1-\eps)^2\gamma B}_{Q_2(s^2,a^{2+})}+\alpha^2\gamma^2(1-\eps)\eps X + \alpha \gamma \eps X^{\prime\prime}
    \end{split}
\end{equation}
where 
\begin{equation}
    \begin{split}
        0&\leq X \leq Q_1(s^1,a^{1+}) = \alpha(1-\eps)B, \\
        0&\leq X^\prime \leq Q_2(s^1,a^{1+}) \leq  \alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha^2 \gamma \eps(1-\eps)B = \alpha(1-\eps)(2-\alpha +\alpha\gamma\eps)B, \\
        0&\leq X^{\prime\prime} \leq Q_2(s^2,a^{2+}) = \alpha^2(1-\eps)^2\gamma B. 
    \end{split}
\end{equation}
In the sparse setting \eqref{eq:sparse_reward}, $r(s^1,a^{1+},s_a) = B$ when $s_a=s_{T^+}$ and $r(s^2,a^{2+},s_a) = 0$. Now we check Claim 1, Claim 2, and Claim 3 for $k=2$.\\
{\bf Claim 1:} $Q_{k+1}(s^d,a^{d+})> Q_{k}(s^d,a^{d+}),\;\forall d\in\bb N^+, d\leq k$. For $d=1$:
\begin{equation}
    \begin{split}
        &Q_3(s^1,a^{1+})>Q_2(s^1,a^{1+})\\
        \iff&\alpha(1-\alpha)^2(1-\eps)B-\alpha^2\gamma\eps X+\alpha\gamma\eps X^\prime>0\\
        \impliedby & (1-\alpha)^2(1-\eps)B\overset{(i)}{>}\alpha^2\gamma\eps(1-\eps)B \iff \eps < \frac{(1-\alpha)^2}{\alpha^2\gamma},
    \end{split}
\end{equation}
where inequality $(i)$ follows $ X^\prime\geq 0$ and $X\leq \alpha (1-\eps)B)$. The above condition $\eps < {(1-\alpha)^2}/{\alpha^2\gamma}$ is automatically satisfied, since $\alpha$ is generally small in practice ($\alpha\leq 0.5$), hence the condition $ (1-\alpha)^2/\alpha^2\gamma>1$ and the above inequality holds since $\eps<1/2$ (by Assumption \ref{assump:transit_mat}). For $d = 2$, $ Q_3(s^2,a^{2+})>Q_2(s^2,a^{2+})$ is directly obtained by \eqref{eq:Q32Calculate}. Hence, Claim 1 is verified.\\
{\bf Claim 2:} $Q_{k}(s^{d^\prime},a^{d^\prime+})>Q_{k}(s^d,a^{d+}),\;\forall d^\prime \in \bb N^+, d^\prime<d\leq k$. 
\begin{equation}
    \begin{split}
        Q_2(s^1,a^{1+}) &= \alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X\\
        &\geq \alpha(1-\eps)B > \alpha^2(1-\eps)^2\gamma B=Q_2(s^2,a^{2+})
    \end{split}
\end{equation}
{\bf Claim 3:} $Q_{k}(s^d,a^{d+})> Q_{k}(s^d,a^{d-}),\; \forall d\in\bb N^+, d\leq k$. For $d=2$ 
\begin{equation}
    Q_2({s^2,a^{2+}}) = \alpha^2(1-\eps)^2\gamma B >0 = Q_2({s^2,a^{2-}}).
\end{equation}
For $d=1$,
\begin{equation}
    Q_2(s^1,a^{1+}) =  \alpha(1-\alpha)(1-\eps)B+\alpha(1-\eps)B + \alpha \gamma \eps X > a(1-\eps)B>\alpha^2 \gamma (1-\eps)B \geq Q_2(s^1,a^{1-}),
\end{equation}
hence, Claim 3 is verified.

\paragraph{Induction.} Next, we assume Claim 1, Claim 2, and Claim 3 hold for an integer $k\geq2$, we will use induction to show Claim 1, Claim 2, and Claim 3 hold for $k+1$. Notice that the agent will receive reward $B$ upon the arrival of $s_{T+}$, we distinguish the cases between $d\geq 2$ and $d=1$, for the different Q learning update. 
\sz{editing assumption, will need to adjust the whole proof a bit.}\\
{\bf Claim 1:} $Q_{k+1}(s^d,a^{d+})> Q_{k}(s^d,a^{d+}),\;\forall d\in\bb N^+, 2\leq d\leq k$.
\begin{equation}
    \begin{split}
        &Q_{k+1}(s^d,a^{d+})>Q_{k}(s^d,a^{d+})\\
        \iff & (1-\alpha)Q_k(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_k(s^{d-1},a^{(d-1)+})+\alpha \gamma \eps X>Q_k(s^d,a^{d+})\\
        \impliedby & \alpha\gamma(1-\eps) Q_k(s^{d-1},a^{(d-1)+})\overset{(i)}{>}\alpha Q_{k }(s^d,a^{d+}) \impliedby  \gamma(1-\eps)\overset{(ii)}{>}1 \\
        \iff & \eps  <(1-\gamma)/\gamma,
    \end{split}
\end{equation}
where inequality $(i)$ follows $0\leq X\leq Q_{k}(s^d,a^{d+}))$ and inequality $(ii)$ follows $Q_k(s^{d-1},a^{(d-1)+})>Q_{k}(s^d,a^{d+})$. 
    \sz{writing here, adding $d=1$}
When $d=1$, we have    
    
\begin{equation}
    \begin{split}
        &Q_{k+1}(s^1,a^{1+})>Q_{k}(s^1,a^{1+})\\
        \iff & (1-\alpha)Q_k(s^1,a^{1+})+\alpha(1-\eps)B+\alpha \gamma \eps X^\prime>Q_k(s^1,a^{1+})\\
        \impliedby & \alpha\gamma(1-\eps) Q_k(s^{1},a^{1+})\overset{(i)}{>}\alpha Q_{k }(s^d,a^{d+}) \impliedby  \gamma(1-\eps)\overset{(ii)}{>}1 \\
        \iff & \eps  <(1-\gamma)/\gamma,
    \end{split}
\end{equation}
    
Hence, Claim 1 is verified since $(1-\gamma)/\gamma>(1-\alpha)(1-\gamma)/\gamma$.\\
{\bf Claim 2:} $Q_{k}(s^{d^\prime},a^{d^\prime+})>Q_{k}(s^d,a^{d+}),\;\forall d^\prime \in \bb N^+, d^\prime<d\leq k$. Notice that
\begin{equation}
    \label{eq:QValue_update_claim2}
    \begin{split}
        Q_{k+1}(s^d,a^{d+})& = (1-\alpha)Q_{k}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+})+\alpha\gamma\eps X^\prime\\
        Q_{k}(s^d,a^{d+})& = (1-\alpha)Q_{k-1}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k-1}(s^{d-1},a^{(d-1)+})+\alpha\gamma\eps X^{\prime\prime}\\ Q_{k+1}(s^{d^\prime},a^{d^\prime+})& = (1-\alpha)Q_{k}(s^{d^\prime},a^{d^\prime+})+\alpha\gamma(1-\eps)Q_{k}(s^{d^\prime-1},a^{(d^\prime-1)+})+\alpha\gamma\eps X^{\prime\prime\prime},
    \end{split}
\end{equation}
where $0\leq X^\prime \leq Q_k(s^d,a^{d+})$, $0\leq X^{\prime\prime} \leq Q_{k-1}(s^{d},a^{d+})$, and $0\leq X^{\prime\prime\prime} \leq Q_k(s^{d^\prime},a^{d^\prime+})$. Hence
\begin{equation}
    \begin{split}
        &Q_{k+1}(s^{d^\prime},a^{d^\prime+})>Q_{k+1}(s^d,a^{d+})\\
        \impliedby & (1-\alpha)Q_{k}(s^{d^\prime},a^{d^\prime+})+\alpha\gamma(1-\eps)Q_{k}(s^{d^\prime-1},a^{(d^\prime-1)+})\\
        & \overset{(i)}{>} (1-\alpha+\alpha\gamma\eps)Q_{k}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+})\\
        \impliedby & (1-\alpha)Q_{k}(s^{d^\prime},a^{d^\prime+}) \overset{(ii)}{>} (1-\alpha+\alpha\gamma\eps)Q_{k}(s^d,a^{d+})\\
        \impliedby & (1-\alpha)Q_{k}(s^{d^\prime},a^{d^\prime+}) \qquad (\text{plug in } Q_k(s^d,a^{d+}) \text{ from } \eqref{eq:QValue_update_claim2}) \\
        & > (1-\alpha+\alpha\gamma\eps)\left[(1-\alpha)Q_{k-1}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k-1}(s^{d-1},a^{(d-1)+})+\alpha\gamma\eps X^{\prime\prime} \right]\\
        \impliedby &  (1-\alpha)Q_{k}(s^{d^\prime},a^{d^\prime+}) \overset{(iii)}{>}(1-\alpha +\alpha\gamma\eps)\left[(1-\alpha+\alpha\gamma\eps)Q_{k-1}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k-1}(s^{d-1},a^{(d-1)+})\right]\\
        \impliedby & \frac{(1-\alpha)}{(1-\alpha+\alpha\gamma)}\overset{(iv)}{>}(1-\alpha +\alpha\gamma\eps) \iff \eps <\frac{(1-\gamma)(1-\alpha)}{\gamma(1-\alpha+\alpha\gamma)},
    \end{split}
\end{equation}
where inequality $(i)$ follows $Q_k(s^d,a^{d+})>Q_k(s^d,a^{d-}),Q_k(s^{d+1},a^{(d+1)+})$, $(ii)$ follows $Q_{k}(s^{d^\prime-1},a^{(d^\prime-1)+})>Q_{k}(s^{d-1},a^{(d-1)+})$, inequality $(iii)$ follows $X^{\prime\prime}\leq Q_{k-1}(s^d,a^{d+}))$, and inequality $(iv)$ follows $Q_{k-1}(s^d,a^{d+}))>Q_{k-1}(s^d,a^{d+})),Q_{k-1}(s^{d-1},a^{(d-1)+})))$. Hence, Claim 2 is verified since $\frac{(1-\gamma)(1-\alpha)}{\gamma(1-\alpha+\alpha\gamma)}>\frac{(1-\alpha)(1-\gamma)}{\gamma}$.\\
{\bf Claim 3:} $Q_{k}(s^d,a^{d+})> Q_{k}(s^d,a^{d-}),\; \forall d\in\bb N^+, d\leq k$. Notice that
\begin{equation}
    \label{eq:QValue_update_claim3}
    \begin{split}
        Q_{k+1}(s^d,a^{d-})& \leq  (1-\alpha)Q_{k}(s^d,a^{d-})+\alpha\gamma Q_{k}(s^{d},a^{d+})\\
        Q_{k}(s^d,a^{d-})& \leq (1-\alpha)Q_{k-1}(s^d,a^{d-})+\alpha\gamma Q_{k-1}(s^{d},a^{d+})\\
        Q_{k+1}(s^d,a^{d+})& = (1-\alpha)Q_{k}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+})+\alpha\gamma\eps X^{\prime\prime}
    \end{split}
    \end{equation}
    where $0\leq X^{\prime\prime} \leq Q_{k}(s^{d},a^{d+})$.
\begin{equation}
    \begin{split}
        &Q_{k+1}(s^d,a^{d+})>Q_{k+1}(s^d,a^{d-})\\
        \impliedby & (1-\alpha)Q_{k}(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+}) \overset{(i)}{>} (1-\alpha)Q_{k}(s^d,a^{d-})+\alpha\gamma Q_{k}(s^{d},a^{d+})\\
        \iff & (1-\alpha-\alpha\gamma)Q_{k}(s^d,a^{d+}) + \alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+}) >  (1-\alpha)Q_{k}(s^d,a^{d-})\\
        \impliedby & (1-\alpha-\alpha\gamma)Q_{k}(s^d,a^{d+}) + \alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+})\qquad (\text{plug in } Q_k(s^d,a^{d-}) \text{ from } \eqref{eq:QValue_update_claim3})\\
        &>(1-\alpha)\left[(1-\alpha)Q_{k-1}(s^d,a^{d-})+\alpha\gamma Q_{k-1}(s^{d},a^{d+})\right]\\
          \impliedby & (1-\alpha-\alpha\gamma)Q_{k}(s^d,a^{d+}) + \alpha\gamma(1-\eps)Q_{k}(s^{d-1},a^{(d-1)+})\overset{(ii)}{>}(1-\alpha)\left[(1-\alpha)Q_{k-1}(s^d,a^{d-})+\alpha\gamma Q_{k}(s^{d},a^{d+})\right]\\
        \iff & (1-\alpha-2\alpha\gamma+\alpha^2\gamma)Q_k(s^d,a^{d+})+\alpha\gamma(1-\eps)Q_k(s^{d-1},a^{(d-1)+}) > (1-\alpha)^2Q_{k-1}(s^d,a^{d-})\\
        \impliedby & (1-\alpha-2\alpha\gamma+\alpha^2\gamma)+ \alpha\gamma(1-\eps)\overset{(iii)}{>}(1-\alpha)^2 \iff \eps < \frac{(1-\alpha)(1-\gamma)}{\gamma},
    \end{split}
\end{equation}
where inequality $(i)$ follows $X^{\prime\prime} \geq 0$, inequality $(ii)$ follows $Q_{k}(s^d,a^{d+})>Q_{k-1}(s^d,a^{d+})$, and inequality $(iii)$ follows $Q_{k}(s^d,a^{d+}),Q_{k}(s^{d-1},a^{(d-1)+})>Q_{k-1}(s^d,a^{d-})$. Hence, Claim 3 is verified. We shall note the the derivation for $d=1$ is slightly different, since one also need to consider the reward $B$, but the overall proof strategy and result for the $d=1$ case remains the same. In conclusion, by induction, we know that Claim 1, 2, and 3 hold for any positive integer $k$, which finishes the proof.


\end{proof}

\subsection{Weakly Absorbing States}
Even though we have provided the definition of an optimal Q function, the properties of such optimal Q function remains vague. To better understand the optimal Q function, we will next introduce the {\em weakly absorbing states}.

\begin{definition}[Weakly Absorbing States]
    \label{def:WeaklyAbsorb}
    Given an MDP $\mc M = (\mc S,\mc A, P, r, \gamma)$ satisfying Assumption \ref{assump:transit_mat}-\ref{assump:min_step_correct_step}, with Q function $Q(\cdot,\cdot)$, we say a state $s^\prime\in \mc S$ is {\em weakly absorbing} with {\em absorbing radius} $R$ if $\forall s^\prime\in \mc S$, such that $D(s,s^\prime)\leq R$, the subsequent state $s_a$ of $s$ after taking a greedy action
    \begin{equation*}
         a=\underset{a^\prime\in \mc A}{\arg\max}\;Q(s,a^\prime).
    \end{equation*}
    satisfies $D(s_a,s^\prime) = D(s,s^\prime) - 1$ with probability $1-\eps$.
\end{definition}
\paragraph{Connection Between Weakly Absorbing States and Optimal Q functions.}
In traditional MDP, an absorbing state $s^\prime$ is the states that only transit to itself. As for the a weakly absorbing state $s^\prime$ in our setting, all other states $s$ move one step closer to $s^\prime$ with probability $1-\eps$ if the action is taken greedily at state $s$. Recall the definition of an optimal Q function (Definition \ref{def:OptimalCondPracRL}), one may found that, if $s^\prime \in \underset{s\in \mc S_{T^+}}{\arg\min}\mc D(s_0,s)$ ($s^\prime$ is closest desired terminal state to the initial state $s_0$) is a weakly absorbing state with radius $D(s_0,s^\prime)$, then the action $a_0$ taken greedily will be correct ($a_0\in \mc A^+(s_0)$) and thus $a_1$ taken at $s_1$ will still be correct ($a_1\in \mc A^+(s_1)$) with probability at least $1-\eps$. However, even if the agent takes a correct action at $s_0$, $s_1$ may not necessarily be one step closer to $s^\prime$, due to the randomness of the transition matrix $\mb P$. Intuitively, we state the connection between the radius $R$ of the weakly absorbing state $s^\prime$ as follows:
\begin{center}
    \em Given an $\mc M = (\mc S,\mc A, P, r, \gamma)$ satisfying Assumption \ref{assump:transit_mat}-\ref{assump:min_step_correct_step}, with the initial state $s_0$ and a Q function $Q(\cdot,\cdot)$. If $\forall s^\prime \in \underset{s\in \mc S_{T^+}}{\arg\min}\mc D(s_0,s)$, $s^\prime$ is a weakly absorbing state with radius $R\geq D(s_0,\mc S_{T^+})$, the probability of $Q(\cdot,\cdot)$ being an optimal Q function increases with larger $R$. 
\end{center}
When we have the largest possible radius $R$, we can conclude a sufficient condition of an optimal Q function:
\begin{center}
    \em  Given an $\mc M = (\mc S,\mc A, P, r, \gamma)$ satisfying Assumption \ref{assump:transit_mat}-\ref{assump:min_step_correct_step}, with the initial state $s_0$ and a Q function $Q(\cdot,\cdot)$. If $\forall s^\prime \in \underset{s\in \mc S_{T^+}}{\arg\min}\mc D(s_0,s)$, $s^\prime$ is a weakly absorbing state with radius $R=\underset{s\in reach_{\mc M}(s_0)}{\max} D(s,\mc S_{T^+})$, then $Q(\cdot,\cdot)$ is an optimal Q function of $\mc M$ with probability 1.
\end{center}


\begin{lemma}[$Q_k(s,a)$ with Intermediate Rewards Setting (c)]
\label{lemma:Qk_bounds_induction_IR_c}
Let $\mc M = (\mc S,\mc A, P, r, \gamma)$ be an MDP with desired terminal states $\mc S_{T^+}$ and intermediate states $\mc S_{I} = \{s_{i_1},s_{i_2},\dots,s_{i_n}\}$. Suppose $\mc M$ satisfies Assumption \ref{assump:transit_mat}, \ref{assump:min_step_correct_step}, \ref{assump:IntermediateStates}, \ref{assump:diff_settings_IS} (c), and \ref{assump:min_dist_IS} if the reward function $r(\cdot)$ follows the intermediate reward setting \eqref{eq:intermediate_reward_setting} and the Q function is zero-initialized \eqref{eq:Q-learning_zero_init}. Then $
Q_k(s,a)$ after $k$ iteration of synchronous Q-learning \eqref{eq:SyncQLearningValue} satisfies the following properties
\begin{align}   
    \label{eq:def_qj_func}
    q^{(j)}(k,d) =& \begin{cases}
        \left[\sum_{i=0}^{k-d}\binom{i+d-1}{d-1}(1-\alpha)^i\right]\alpha^{d}\gamma^{d-1}B_{I_j}, & \forall k,d\in \bb N^+, d\leq k,\;\forall j \in [N+1],\\
        0, & \text{otherwise},\\    
        \end{cases}
\end{align}
where we also slightly abuse the notation by assuming $B_{I_{N+1}} = B$. In addition, $\forall j \in \mc I_d(s)$, let $\mc A_j^+(s)$ denote the set of actions that take the state $s$ one step forward to $s_{i_j}$:
\begin{equation}
    \label{eq:ActionToS_i_j}
    D(s_a,s_{i_j}) = D(s,s_{i_j})-1,\;\forall a_j \in \mc A_j^+(s),
\end{equation}
where $s_a$ is the subsequent state of state action pair $(s,a)$. Let $\mc I_m(s)$ denote all indices of $j^\star$ that constitute the maximization definition of $V_k(s)$:
\begin{equation}
    \label{eq:def_Im(s)}
    V_k(s) = \max_{j\in \mc I_d(s)}\left\{q^{(j)}(k,d_j)+\eta\paren{k,d_j;\mc I_d(s_{i_j})}\right\} = q^{(j^\star)}(k,d_{j^\star})+\eta\paren{k,d_{j^\star};\mc I_d(s_{i_{j^\star}})},\;\forall j^\star \in \mc I_m(s)
\end{equation}
then we also have 
\begin{equation}
    \label{eq:argmaxQ_j=V}
        q^{(j^\star)}(k,d_{j^\star})+\eta\paren{k,d_{j^\star};\mc I_d(s_{i_{j^\star}})}= V_k(s) = Q_k(s,a_{j^\star}),\;\forall a_{j^\star}\in \mc A_{j^\star}^+(s),
\end{equation}
in words, if an index $j^\star\in \mc I_m(s)$ maximizes $q^{(j)}(k,d_j)+\eta\paren{k,d_j;\mc I_d(s_{i_j})}$, then $\forall a_{j^\star}\in \mc A_{j^\star}^+(s)$, $a_{j^\star}$ is also the maximizer of $\max_{a\in \mc A}Q_k(s,a)$ (or equivalently $Q_k(s,a_{j^\star}) = V_k(s)$).

\end{lemma}


\begin{lemma}[$Q_k(s,a)$ with Intermediate Rewards Setting (c)]
\label{lemma:Qk_bounds_induction_IR_c}
Let $\mc M = (\mc S,\mc A, P, r, \gamma)$ be an MDP with desired terminal states $\mc S_{T^+}$ and intermediate states $\mc S_{I} = \{s_{i_1},s_{i_2},\dots,s_{i_n}\}$. Suppose $\mc M$ satisfies Assumption \ref{assump:transit_mat}, \ref{assump:min_step_correct_step}, \ref{assump:IntermediateStates}, \ref{assump:diff_settings_IS} (c), and \ref{assump:UncorrelatedDRIS} if the reward function $r(\cdot)$ follows the intermediate reward setting \eqref{eq:intermediate_reward_setting} and the Q function is zero-initialized \eqref{eq:Q-learning_zero_init}. Then $V_k(s)$ the value function at state $s$ after $k$ iteration of synchronous Q-learning \eqref{eq:SyncQLearningValue} satisfies the following recursive definition: 
\begin{equation}
    \label{eq:DPVk_settingc}
    \begin{split}
        V_k(s) &= \max_{j\in \mc I_d(s)}\left\{q^{(j)}(k,d_j)+\eta\paren{k,d_j;\mc I_d(s_{i_j})}\right\},\\
        \eta\paren{k,d_j;\mc I_d(s_{i_j})} &=
        \begin{cases}
            \underset{j^\prime \in \mc I_d(s_{i_j})}{\max}\left\{q^{(j^\prime)}(k,d_j+d_{j,j^\prime})+\eta\paren{k,d_j+d_{j,j^\prime};\mc I_d(s_{i_{j^\prime}})}\right\},&\text{ if }\;s_{i_j}\notin \mc S_{T^+},\\
            0,&\text{ if }\;s_{i_j}\in \mc S_{T^+},
        \end{cases} 
    \end{split}
\end{equation}
where 
\begin{equation}
    d_j = D(s,s_{i_j}),\;d_{j,j^\prime} = D(s_{i_j},s_{i_{j^\prime}}),\;d_{j,T^+}=D(s_{i_j},s_{T^+}),
\end{equation}
and
\begin{align}   
    \label{eq:def_qj_func}
    q^{(j)}(k,d) =& \begin{cases}
        \left[\sum_{i=0}^{k-d}\binom{i+d-1}{d-1}(1-\alpha)^i\right]\alpha^{d}\gamma^{d-1}B_{I_j}, & \forall k,d\in \bb N^+, d\leq k,\;\forall j \in [N+1],\\
        0, & \text{otherwise},\\    
        \end{cases}
\end{align}
where we also slightly abuse the notation by assuming $B_{I_{N+1}} = B$. In addition, $\forall j \in \mc I_d(s)$, let $\mc A_j^+(s)$ denote the set of actions that take the state $s$ one step forward to $s_{i_j}$:
\begin{equation}
    \label{eq:ActionToS_i_j}
    D(s_a,s_{i_j}) = D(s,s_{i_j})-1,\;\forall a_j \in \mc A_j^+(s),
\end{equation}
where $s_a$ is the subsequent state of state action pair $(s,a)$. Let $\mc I_m(s)$ denote all indices of $j^\star$ that constitute the maximization definition of $V_k(s)$:
\begin{equation}
    \label{eq:def_Im(s)}
    V_k(s) = \max_{j\in \mc I_d(s)}\left\{q^{(j)}(k,d_j)+\eta\paren{k,d_j;\mc I_d(s_{i_j})}\right\} = q^{(j^\star)}(k,d_{j^\star})+\eta\paren{k,d_{j^\star};\mc I_d(s_{i_{j^\star}})},\;\forall j^\star \in \mc I_m(s)
\end{equation}
then we also have 
\begin{equation}
    \label{eq:argmaxQ_j=V}
        q^{(j^\star)}(k,d_{j^\star})+\eta\paren{k,d_{j^\star};\mc I_d(s_{i_{j^\star}})}= V_k(s) = Q_k(s,a_{j^\star}),\;\forall a_{j^\star}\in \mc A_{j^\star}^+(s),
\end{equation}
in words, if an index $j^\star\in \mc I_m(s)$ maximizes $q^{(j)}(k,d_j)+\eta\paren{k,d_j;\mc I_d(s_{i_j})}$, then $\forall a_{j^\star}\in \mc A_{j^\star}^+(s)$, $a_{j^\star}$ is also the maximizer of $\max_{a\in \mc A}Q_k(s,a)$ (or equivalently $Q_k(s,a_{j^\star}) = V_k(s)$).

\end{lemma}
\begin{remark}[The Stopping Condition of Recursion \eqref{eq:DPVk_settingc}]
\label{remark:StopCondRecSettingC}
Note that the recursion  \eqref{eq:DPVk_settingc} ends once $s_{i_j^\star}\in \mc S_{T^\star}$, and this will eventually happens because Assumption \ref{assump:IntermediateStates} guarantees that $s_{i_{j^\star}}$ is not reachable from $s_{i_{j^\star}}$, which implies $[N+1]\backslash{j^\star}$, the superset of $\mc I_d(s_{i_j})$ is shrinking in the recursion. 
\end{remark}
\begin{proof}
We will use induction to prove the conditions \eqref{eq:DPVk_settingc} and \eqref{eq:argmaxQ_j=V}. 

\paragraph{Intuition.}
The proof of \eqref{eq:DPVk_settingc} and \eqref{eq:argmaxQ_j=V} follows the following rough argument. We will show that, for an index $j^\star\in \mc I_m(s)$ ($j^\star$ may not be unique) such that $q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})}$ is the largest:
\begin{equation}
    \begin{split}
        V_k(s) &= \max_{j\in \mc I_{d}(s)}\left\{q^{(j)}(k,D(s,s_{i_j})) +\eta\paren{k,D(s,s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})},
    \end{split}
\end{equation}
then after moving one step forward to the intermediate state $s_{i_{j^\star}}$ by taking action $a_{j^\star}\in \mc A_{j^\star}^+(s)$. {\em If $s_{a_{j^\star}}$ is not the intermediate state} ($s_{a_{j^\star}}\neq s_{i_{j^\star}}$), then $q^{(j^\star)}(k,D(s_{a_{j^\star}},s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})}$ of the subsequent state $s_{a_{j^\star}}$ is still the largest: 
\begin{equation}
    \begin{split}
        V_k(s_{a_{j^\star}}) &= \max_{j\in \mc I_{d}(s_{a_{j^\star}})}\left\{q^{(j)}(k,D(s_{a_{j^\star}},s_{i_j})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^\star)}(k,D(s_{a_{j^\star}},s_{i_{j^\star}})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})}\\
        &= q^{(j^\star)}(k,D(s,s_{i_{j^\star}})-1) +\eta\paren{k,D(s,s_{i_{j^\star}})-1;\mc I_d(s_{i_{j^\star}})}.
    \end{split}
\end{equation}
{\em If $s_{a_{j^\star}}$ is the intermediate state $s_{i_{j^\star}}$ ($s_{a_{j^\star}}=s_{i_{j^\star}}$)}, we have
\begin{equation}
    \begin{split}
        V_k(s_{i_{j^\star}}) &= \max_{j^\prime\in \mc I_{d}(s_{i_{j^\star}})}\left\{q^{(j)}(k,D(s_{i_{j^\star}},s_{i_{j^\prime}})) +\eta\paren{k,D(s_{i_{j^\star}},s_{i_{j^\prime}});\mc I_d(s_{i_{j^\star}})}\right\},
    \end{split}
\end{equation}
which justifies the recursive definition \eqref{eq:DPVk_settingc} and condition \eqref{eq:argmaxQ_j=V}. We will first prove the following claim:
\begin{claim}[Property of $j^\star$.]
\label{claim:jstar_maximizer_property}
Recall the definition of $\mc I_m(s)$ \eqref{eq:def_Im(s)}, $\forall j^\star\in \mc I_m(s)$, $\forall a_{j^\star}\in \mc A_{j^\star}^+(s)$, we have $j^\star\in \mc I_m(s_{a_{j^\star}})$, 
namely:
\begin{equation}
    \label{eq:jstar_property}
    j^\star \in \underset{j\in \mc I(s_{a_{j^\star}})}{\arg\max}\left\{q^{(j)}(k,D(s_{a_{j^\star}},s_{i_j})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_j});\mc I_d(s_{i_{j}})}\right\},
\end{equation}
where $s_{a_{j^\star}}$ is the subsequent state of state action pair $(s,a_{j^\star})$.
\end{claim}
Lemma \ref{lemma:Qk_bounds_value_SR} implies that $q^{(j)}(k,d)$ is monotonic decreasing as $d$ increases, so $\eta\paren{k,d;\mc I_d(s_{i_{j}})}$ is also monotonic decreasing while $d$ increases, as the recursion \eqref{eq:DPVk_settingc} for $\eta\paren{k,D(s,s_{i_{j}});\mc I_d(s_{i_{j}})}$ can be essentially written as
\begin{equation*}
    \begin{split}
        \eta\paren{k,D(s,s_{i_{j}});\mc I_d(s_{i_{j}})} =\;& q^{(j)}(k,D(s,s_{i_{j}}))+q^{(j_1)}(k,D(s,s_{i_{j}})+D(s_{i_j},s_{i_{j_1}}))\\
        &+ \dots + q^{(N+1)}(k,D(s,s_{i_{j}})+D(s_{i_j},s_{i_{j_1}})+\dots + D(s_{i_{j_m}},s_{i_{N+1}})),
    \end{split}
\end{equation*}
for some $j,j_1,j_2,\dots,j_m$. Hence, $\forall j\in \mc I_d(s),j\neq j^\star$, we have
\begin{equation}
    \begin{split}
        &q^{(j^\star)}(k,D(s_{a_{j^\star}},s_{i_{j^\star}})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})}\\
        =\;&  q^{(j^\star)}(k,D(s,s_{i_{j^\star}})-1) +\eta\paren{k,D(s,s_{i_{j^\star}})-1;\mc I_d(s_{i_{j^\star}})} \\
        \overset{(i)}{\geq}\;& q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})}\\
        \overset{(ii)}{\geq}\;& q^{(j)}(k,D(s,s_{i_{j}})) +\eta\paren{k,D(s,s_{i_{j}});\mc I_d(s_{i_{j}})}\\
        \overset{(iii)}{\geq}\;&q^{(j)}(k,D(s_{a_{j^\star}},s_{i_{j}})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_{j}});\mc I_d(s_{i_{j}})}.
    \end{split}
\end{equation}
Inequality $(i)$ and $(iii)$ hold by the monotonic decreasing property of $q^{(j)}(k,d)$ and $\eta\paren{k,d;\mc I_d(s_{i_{j}})}$, since Assumption \ref{assump:UncorrelatedDRIS} implies $D(a_{j^\star},s_{i_j})\geq D(a_{j^\star},s_{i_j})$. Note that we use $\geq$ instead of $>$ as stated in Lemma \ref{lemma:Qk_bounds_value_SR} for the case where $k$ is not large enough and $q^{(j)}(k,d)$ could be $0$. Inequality $(ii)$ holds by the assumption that $j^\star$ maximizes $q^{(j)}(k,D(s_{a_{j^\star}},s_{i_j})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_j});\mc I_d(s_{i_{j}})}$ (see \eqref{eq:jstar_property}). Hence, we conclude that $j^\star$ also maximizes $q^{(j)}(k,D(s_{a_{j^\star}},s_{i_{j}})) +\eta\paren{k,D(s_{a_{j^\star}},s_{i_{j}});\mc I_d(s_{i_{j}})}$.


\paragraph{Initial Condition for $k=1$.} 
When $k=1$, since Assumption \ref{assump:IntermediateStates} implies that all intermediate states $s_{i_j}$ are from $\mc S\backslash\mc S_{T^+}$, and combine the deterministic Assumption \ref{assump:transit_mat}, we know that the subsequent state $s_a$ of a state action pair $(s,a)$ cannot be a terminal state and an intermediate state at the same time. Hence, by the Q-learning update \eqref{eq:SyncQLearningValue}, we know that 
\begin{equation}
    Q_1(s,a) = 
    \begin{cases}
        \alpha B_{I_j},&\text{ if } D(s,s_{i_j})=1,\;a\in \mc A^+_j(s),\;\forall (s,a)\in \mc S\times \mc A,\;\forall j\in [N+1],\\
        0,&\text{ otherwise},
    \end{cases}
\end{equation}
which implies that 
\begin{equation}
    \begin{split}
        V_1(s) &= \max_a Q_1(s,a)= \max_{\substack{j\in [N+1],\\{D(s,s_j)=1}}}\alpha B_{I_j}=\max_{j\in \mc I_d(s)}\alpha B_{I_j} \\
        &= \max_{j\in\mc I_d(s)}q^{(j)}(1,1)= \max_{j\in\mc I_d(s)}\{q^{(j)}(1,1)+\eta\paren{1,1;\mc I_d(s_{i_j})}\},
    \end{split}
\end{equation}
where the last equality holds because $\eta\paren{1,1;\mc I_d(s_{i_j})}=0$, as \eqref{eq:def_qj_func} implies $q^{(j)}(1,d) = 0$, when $d>1$. Therefore, we conclude that the initial condition of \eqref{eq:DPVk_settingc} holds. Meanwhile, $\forall j^\star\in \underset{j\in \mc I_d(s)}{\arg\max}\;\alpha B_{I_j}$, we have 
\begin{equation}
    V_1(s) = \alpha B_{I_{j^\star}} = Q_1(s,a_{j^\star}),
\end{equation}
which implies that the initial condition condition of \eqref{eq:argmaxQ_j=V} also holds.
\paragraph{Induction.}
Now suppose the conditions \eqref{eq:DPVk_settingc} and \eqref{eq:argmaxQ_j=V} hold for $k$, we will show they also hold for $k+1$. 
Recall the Q-learning update \eqref{eq:SyncQLearningValue}:
\begin{equation*}
    \begin{split}
            Q_{k+1}(s,a)&=(1-\alpha)Q_{k}(s,a)+\alpha\left(r(s,a,s_a)+\gamma V_k(s_a)\right),\;V_{k}(s_a)=\max_{a\in \mc A}Q_{t}(s,a),\;\forall (s,a)\in \mc S\times \mc A,
    \end{split}
\end{equation*}
where $s_a$ is the subsequent state of state action pair $(s,a)$, we know that 
\begin{equation}
    \label{eq:settingc_QL_update}
    Q_{k+1}(s,a_j) = (1-\alpha)Q_{k}(s,a_j)+\alpha\left(r(s,a_j,s_{a_j})+\gamma V_k(s_{a_j})\right),\;\forall j\in \mc I_d(s),a_j\in \mc A^+_j(s).
\end{equation}
Recall the recursive definition of $V_k(s)$ in \eqref{eq:DPVk_settingc} and the definition of $\mc I_m(s)$ \eqref{eq:def_Im(s)}:
\begin{equation}
    \label{eq:settingc_derivation_Vk}
    \begin{split}
        V_k(s) &= \max_{j\in \mc I_{d}(s)}\left\{q^{(j)}(k,D(s,s_{i_j})) +\eta\paren{k,D(s,s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})},\;\forall j^\star \in \mc I_m(s).
    \end{split}
\end{equation}
Then \eqref{eq:argmaxQ_j=V} implies that
\begin{equation}
    \label{eq:settingc_derivation_Qk}
    Q_k(s,a_{j^\star}) = \max_{a\in \mc A}Q_k(s,a),\;\forall j^\star \in \mc I_m(s),\;\forall a_{j^\star}\in \mc A_{j^\star}^+(s).
\end{equation}
We will discuss the three following cases:

\begin{itemize}
    \item $\min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \geq k+2$;
    \item $\min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) = k+1$;
    \item $2\leq \min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \leq k-1$;
    \item $1 = \min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \leq k-1$.
\end{itemize} 

\paragraph{When $\min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \geq k+2$.} 
\eqref{eq:settingc_derivation_Vk} implies that 
\begin{equation}
    \label{eq:settingc_d_geqk+2_Vk=0}
    \begin{split}
        V_k(s) &= q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})} \overset{(i)}{=} \eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})}\\
        &=\max_{j^\prime \in \mc I_d(s_{i_{j^\star}})}\left\{q^{(j^\prime)}(k,D(s,s_{i_{j^\star}})+D(s_{i_{j^\star}},s_{j^\prime}))+\eta\paren{k,D(s,s_{i_{j^\star}})+D(s_{i_{j^\star}},s_{j^\prime}};\mc I_d(s_{i_{j^\prime}}))\right\}\\
        &\overset{(ii)}{=}\max_{j^\prime \in \mc I_d(s_{i_{j^\star}})}\left\{\eta\paren{k,D(s,s_{i_{j^\star}})+D(s_{i_{j^\star}},s_{j^\prime});\mc I_d(s_{i_{j^\prime}})}\right\}=\dots\overset{(iii)}{=}0,\;\forall j^\star\in \mc I_m(s).
    \end{split}
\end{equation}
Equality $(i)$ holds because \eqref{eq:def_qj_func} implies $q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) = 0$, when $D(s,s_{i_{j^\star}})>k$. Similarly for equality $(ii)$, as $D(s,s_{i_{j^\star}})+D(s_{i_{j^\star}},s_{j^\prime})>D(s,s_{i_{j^\star}})\geq k+2>k$ implies that $q^{(j^\prime)}(k,D(s,s_{i_{j^\star}})+D(s_{i_{j^\star}},s_{j^\prime})) = 0$. Equality $(iii)$ holds since each recursion from equality $(i)$ to equality $(ii)$ will induce a non-negative term $q^{(j)}(k,d)$, with $d>D(s,s_{i_{j^\star}})>k$, which implies that all $q^{(j)}(k,d) = 0$ in the future recursions. 

Now consider the value function $V_k(s_a)$ of the subsequent state $s_a$ of state action pair $(s,a)$, $\forall a\in \mc A$:
\begin{equation}
    \label{eq:settingc_d_geqk+2_Vk(sa)=0}
    \begin{split}
        V_k(s_{a}) &= \max_{j\in \mc I(s_{a})}\left\{q^{(j)}(k,D(s_{a},s_{i_j})) +\eta\paren{k,D(s_{a_{j^*}},s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^*)}(k,D(s_{a},s_{i_{j^*}})) +\eta\paren{k,D(s_a,s_{i_{j^*}});\mc I_d(s_{i_{j^*}})}\overset{(i)}{=} 0,\;\forall j^* \in \mc I_m(s_a),
    \end{split}
\end{equation}
where equality $(i)$ holds by the same reason stated for \eqref{eq:settingc_d_geqk+2_Vk=0}, given
\begin{equation}
    \min_{j^*\in \mc I_d(s_a)}D(s_a,s_{i_j}) \geq \min_{j^*\in \mc I_d(s_a)}D(s,s_{i_j})-1 \geq k+1>k.
\end{equation}
Applying the Q-learning update \eqref{eq:SyncQLearningValue} to $Q_k(s,a)$, we have:
\begin{equation}
    \label{eq:settingc_d_geqk+2_Qk(sa)=0}
    \begin{split}
        Q_{k+1}(s,a) &= (1-\alpha)Q_{k}(s,a) + \alpha(r(s,a,s_{a})+\gamma V_k(s_a))\\
        &\overset{(i)}{=}(1-\alpha)Q_{k}(s,a)+\alpha r(s,a,s_a)\\
        &\overset{(ii)}{=}(1-\alpha)Q_{k}(s,a)\leq(1-\alpha)V_k(s) \overset{(iii)}{=} 0, \;\forall a\in \mc A,
    \end{split}
\end{equation}
where equality $(i)$ holds because \eqref{eq:settingc_d_geqk+2_Vk(sa)=0} implies $V_k(s_a) = 0$, equality $(ii)$ holds because $\min_{j\in \mc I_d(s)}D(s,s_{i_j})\geq k+2>1$ implies $s_a\notin \mc S_I$, hence according to the setting of intermediate rewards \eqref{eq:intermediate_reward_setting}, we know $r(s,a,s_a)=0$, and equality $(iii)$ holds because of \eqref{eq:settingc_d_geqk+2_Vk=0}. Hence, we conclude that 
\begin{equation}
    V_{k+1}(s) = \max_{a\in \mc A}Q_{k+1}(s,a) = 0,
\end{equation}
which matches the induction definition of $V_{k+1}(s)$:
\begin{equation}
    V_{k+1}(s) = 0 = \max_{j\in \mc I_d(s)}\left\{q^{(j)}(k+1,D(s,s_{i_j}))+\eta\paren{k+1,D(s,s_{i_j});\mc I_d(s_{i_j})}\right\} ,
\end{equation}
where the last equality holds by the same reason stated for \eqref{eq:settingc_d_geqk+2_Vk=0}, since $D(s,s_{i_j})\geq k+2>k+1$. Hence, the induction condition of \eqref{eq:DPVk_settingc} is verified. As for the induction condition \eqref{eq:argmaxQ_j=V}, since \eqref{eq:settingc_d_geqk+2_Qk(sa)=0} implies that
\begin{equation}
    Q_{k+1}(s,a_{j^\star}) = 0 = \max_{a\in \mc A} Q_{k+1}(s,a) = V_{k+1}(s),  
\end{equation}
which verifies the induction condition \eqref{eq:argmaxQ_j=V}. Therefore, we conclude the induction conditions \eqref{eq:DPVk_settingc} and \eqref{eq:argmaxQ_j=V} hold when $\min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \geq k+2$.

\paragraph{When $\min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) = k+1$.}
In this case, \eqref{eq:settingc_derivation_Vk} implies that 
\begin{equation}
        V_k(s) = q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})} =0,\;\forall j^*\in \mc I_m(s),
\end{equation}
where the last equality holds for the same reason stated for \eqref{eq:settingc_d_geqk+2_Vk=0} since $D(s,s_{i_{j^\star}})\geq k+1>k$. Hence, $\forall a\in \mc A$, we have
\begin{equation}
    0\leq Q_k(s,a) \leq V_k(s) = 0 \implies Q_k(s,a) = 0. 
\end{equation}
$\forall a\in \mc A$, consider the value function $V_k(s_a)$ of the subsequent state $s_a$ of state action pair $(s,a)$:
\begin{equation}
    \label{eq:settingc_d_=k+1_Vk(sa)}
    \begin{split}
        V_k(s_{a}) &= \max_{j\in \mc I(s_{a})}\left\{q^{(j)}(k,D(s_{a},s_{i_j})) +\eta\paren{k,D(s_{a_{j^*}},s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^*)}(k,D(s_{a},s_{i_{j^*}})) +\eta\paren{k,D(s_a,s_{i_{j^*}});\mc I_d(s_{i_{j^*}})},\;\forall j^*\in \mc I_m(s_a)\\
        &\overset{(i)}{=}\begin{cases}
            \alpha^k\gamma^{k-1}B_{I_j},&\text{ if }s_a = s_{i_j},\\
            0,&\text{otherwise},\\
        \end{cases}
    \end{split}
\end{equation}
where equality $(i)$ holds due to the recursive definition of $V_k(s_a)$. Applying the Q-learning update \eqref{eq:SyncQLearningValue} to $Q_k(s,a)$, we have:
\begin{equation}
    \label{eq:settingc_d_=k+1_Qk(sa)=0}
    \begin{split}
        Q_{k+1}(s,a) &= (1-\alpha)Q_{k}(s,a) + \alpha(r(s,a,s_{a})+\gamma V_k(s_a))\\
        &\overset{(i)}{=}(1-\alpha)Q_{k}(s,a)+\alpha \gamma V_k(s_a)\\
        &\overset{(ii)}{=}\alpha\gamma V_k(s_a)\\
        &\overset{(iii)}{=}\begin{cases}
            \alpha^{k+1}\gamma^{k}B_{I_j},&\text{ if }s_a = s_{i_j},\\
            0,&\text{otherwise}.\\
        \end{cases}
    \end{split}
\end{equation}
Equality $(i)$ holds because $\min_{j\in \mc I_d(s)}D(s,s_{i_j}) = k+1>1$ implies $s_a\notin \mc S_I$, hence according to the setting of intermediate rewards \eqref{eq:intermediate_reward_setting}, we know $r(s,a,s_a)=0$, and equality $(iii)$ holds by \eqref{eq:settingc_d_=k+1_Vk(sa)}. Hence, we know that 
\begin{equation}
    \label{eq:settingc_d_=k+1_Vk+1(sa)}
    \begin{split}
        V_{k+1}(s) &= \max_{a\in \mc A}Q_{k+1}(s,a) = \max_{j\in \mc I_d(s)}\alpha^{k+1}\gamma^k B_{I_j}\\
        &=\max_{j\in \mc I_d(s)}\left\{q^{(j)}(k+1,D(s,s_{i_j}))+\eta\paren{k+1,D(s,s_{i_j});\mc I_d(s_{i_j})}\right\},
    \end{split}
\end{equation}
which verifies the induction condition \eqref{eq:DPVk_settingc}. Moreover, from the above equation of $V_{k+1}(s)$, we also have
\begin{equation}
    \begin{split}
        V_{k+1}(s) &= \max_{j\in \mc I_d(s)}\left\{q^{(j)}(k+1,D(s,s_{i_j}))+\eta\paren{k+1,D(s,s_{i_j});\mc I_d(s_{i_j})}\right\}\\
        &= q^{(j^\star)}(k+1,D(s,s_{i_{j^\star}}))+\eta\paren{k+1,D(s,s_{i_j});\mc I_d(s_{i_{j^\star}})}\\
        &= \alpha^{k+1}\gamma^k B_{I_{j^\star}} = Q_{k+1}(s,a_{j^\star}),\;\forall j^\star\in\mc I_m(s),
    \end{split}
\end{equation}
which verifies the induction condition \eqref{eq:argmaxQ_j=V}. we conclude the induction conditions \eqref{eq:DPVk_settingc} and \eqref{eq:argmaxQ_j=V} hold when $\min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) = k+1$.

\paragraph{When $2\leq \min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \leq k-1$.} By the recursive definition of $V_k(s)$, we have  
\begin{equation}
    \begin{split}
        V_k(s) &= \max_{j\in \mc I_{d}(s)}\left\{q^{(j)}(k,D(s,s_{i_j})) +\eta\paren{k,D(s,s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^\star)}(k,D(s,s_{i_{j^\star}})) +\eta\paren{k,D(s,s_{i_{j^\star}});\mc I_d(s_{i_{j^\star}})},\;\forall j^\star \in \mc I_m(s).
    \end{split}
\end{equation}
$\forall a \in \mc A$, we consider the value function $V_k(s_a)$ of $s_a$ (the subsequent state of $(s,a)$) of different action set: $\mc A_j^+(s),\;\forall j\in \mc I_d(s)$ and $\mc A\backslash( \cup_{j\in \mc I_d(s)} \mc A^+(s))$. Then from the recursive definition \ref{eq:DPVk_settingc}, we have
\begin{equation}
    \begin{split}
        V_k(s_a) &= \max_{j\in \mc I(s_{a})}\left\{q^{(j)}(k,D(s_{a},s_{i_j})) +\eta\paren{k,D(s_{a_{j^*}},s_{i_j});\mc I_d(s_{i_{j}})}\right\}\\
        &= q^{(j^*)}(k,D(s_{a},s_{i_{j^*}})) +\eta\paren{k,D(s_a,s_{i_{j^*}});\mc I_d(s_{i_{j^*}})},\;\forall j^*\in \mc I_m(s_a).
    \end{split}
\end{equation}
Then the Q-learning update of state action pair $Q_{k+1}(s,a)$ implies
\begin{equation}
    \begin{split}
        Q_{k+1}(s,a) &= (1-\alpha)Q_k(s,a)+\alpha(r(s,a,s_a)+\gamma V_k(s_a))\overset{(i)}{=}(1-\alpha)Q_k(s,a)+\alpha\gamma V_k(s_a)\\
        &=(1-\alpha)Q_k(s,a) + q^{(j^*)}(k,D(s_{a},s_{i_{j^*}})) +\eta\paren{k,D(s_a,s_{i_{j^*}});\mc I_d(s_{i_{j^*}})},\;\forall j^*\in \mc I_m(s_a)
    \end{split}
\end{equation}

\paragraph{When $1 = \min_{j\in \mc I_d(s)} D(s,s_{i_{j}}) \leq k-1$.}

\sz{writing here}

\section{Auxiliary Results}
\subsection{}
\begin{lemma}
\label{lemma:Qk_bounds_value_SR}
Given a function $q(k,d):\bb N^+\times \bb N^+ \mapsto \bb R^+$ defined as:
\begin{align}
    &q(k,d) = \begin{cases}
        \left[\sum_{i=0}^{k-d}\binom{i+d-1}{d-1}(1-\alpha)^i\right]\alpha^d\gamma^{d-1}B, & \forall k,d\in \bb N^+, d\leq k,\\
        0, & \text{otherwise},\\    
        \end{cases}
\end{align}
we have 
\begin{equation}
    \begin{split}
        q(k,d+1)<q(k,d)\;\forall d\leq k
    \end{split}
\end{equation}
\end{lemma}
\begin{proof}
\paragraph{Proving $q(k,d+1)<q(k,d)$, when $d\leq k-2$.}
Notice that 
\begin{equation}
    \label{eq:qu-<ql+_derivation1}
    \begin{split}
        &q(k,d+1)<q(k,d)\\
        \iff &\left[\sum_{i=0}^{k-d-1}\binom{i+d}{d}(1-\alpha)^i\right]\alpha^{d+1}\gamma^{d}B<\left[\sum_{i=0}^{k-d}\binom{i+d-1}{d-1}(1-\alpha)^i\right]\alpha^d\gamma^{d-1}B\\
        \iff & \left[\sum_{i=0}^{k-d-1}\binom{i+d}{d}(1-\alpha)^i\right]\alpha\gamma<\sum_{i=0}^{k-d}\binom{i+d-1}{d-1}(1-\alpha)^i\\
        \iff &\left\{1+\sum_{i=1}^{k-d-1}\left[\binom{i+d-1}{d-1}+\binom{i+d-1}{d}\right](1-\alpha)^i\right\}\alpha\gamma\\
        &<\sum_{i=0}^{k-d-1}\binom{i+d-1}{d-1}(1-\alpha)^i+\binom{k-1}{d-1}(1-\alpha)^{k-d}\\
        \iff&\underbrace{\left[\sum_{i=1}^{k-d-1}\binom{i+d-1}{d}(1-\alpha)^i\right]\alpha}_{\Gamma_1}\gamma<\underbrace{\left[\sum_{i=0}^{k-d-1}\binom{i+d-1}{d-1}(1-\alpha)^i\right](1-\alpha\gamma)}_{\Gamma_2}+\binom{k-1}{d-1}(1-\alpha)^{k-d}.
    \end{split}
\end{equation}
Notice that 
\begin{equation}
     \begin{split}
         \Gamma_1 =& \left[\sum_{i=1}^{k-d-1}\binom{i+d-1}{d}(1-\alpha)^i\right]\alpha = \left[\sum_{i=1}^{k-d-1}\binom{i+d-1}{d}(1-\alpha)^i\right][1-(1-\alpha)]\\
         =&\left[\sum_{i=1}^{k-d-1}\binom{i+d-1}{d}(1-\alpha)^i\right] -  \left[\sum_{i=1}^{k-d-1}\binom{i+d-1}{d}(1-\alpha)^{i+1}\right]\\
         =&\left\{(1-\alpha)+\sum_{i=2}^{k-d-1}\left[\binom{i+d-1}{d}-\binom{i+d-2}{d}\right](1-\alpha)^i\right\} -\binom{k-2}{d}(1-\alpha)^{k-d}\\
         =&\left[(1-\alpha)+\sum_{i=2}^{k-d-1}\binom{i+d-2}{d-1}(1-\alpha)^i\right] -\binom{k-2}{d}(1-\alpha)^{k-d}\\
         =&\left[\sum_{i=1}^{k-d-1}\binom{i+d-2}{d-1}(1-\alpha)^i\right] -\binom{k-2}{d}(1-\alpha)^{k-d}\\
         =&\left[\sum_{i=0}^{k-d-2}\binom{i+d-1}{d-1}(1-\alpha)^i\right](1-\alpha)-\binom{k-2}{d}(1-\alpha)^{k-d},
     \end{split}
\end{equation}
hence, we have
\begin{equation}
    \begin{split}
        \Gamma_1\gamma<\left[\sum_{i=0}^{k-d-2}\binom{i+d-1}{d-1}(1-\alpha)^i\right](1-\alpha)\gamma<\left[\sum_{i=0}^{k-d-1}\binom{i+d-1}{d-1}(1-\alpha)^i\right](1-\alpha\gamma)=\Gamma_2.
    \end{split}
\end{equation}
Substituting $\Gamma_1<\Gamma_2$ into \eqref{eq:qu-<ql+_derivation1}, we know that 
\begin{equation}
    q(k,d+1)<q(k,d),\;\forall d\leq k-2.   
\end{equation}
\paragraph{Proving $q(k,d+1)<q(k,d)$, when $d = k-1$.}
In this case, we have
\begin{equation}
    \begin{split}
        q(k,d+1) = \alpha^k\gamma^{k-1}B<[1+d(1-\alpha)]\alpha^{k-1}\gamma^{k-2}B=q(k,d).
    \end{split}
\end{equation}


\paragraph{Proving $q(k,d+1)<q(k,d)$, when $d = k$.}
In this case, $q(k,d+1)<q(k,d)$ obviously holds as
\begin{equation}
    q(k,d+1)=0<\alpha^k\gamma^{k-1}B=q(k,d).
\end{equation}
Hence we conclude that $q(k,d+1)<q(k,d),\;\forall d\leq k$.
\end{proof}


\end{proof}

% The following corollary also demonstrates a sufficient condition of optimal Q-functions, using the correct action set $\mc A^+(s)$.

% \begin{corollary}[A Sufficient Condition of Optimal Q-functions]
% \label{corollary:suff_cond_optimal_Q}
% Given a deterministic MDP (Definition \ref{def:transit_mat}) $\mc M = (\mc S,\mc A, P, r, \gamma)$, with initial state $s_0$ and a Q-function $Q(\cdot,\cdot)$, if $\exists n^\star\in \bb N$, such that all greedy actions $a_{t} \in {\arg\max}_{{a^\prime}}Q(s_t,a^\prime)$ taken after $s_{n^\star}$ are correct:
% \begin{equation}
%     a_{t} \in \mc A^+(s_t),\;\forall t\geq n^\star, 
% \end{equation}
% then the Q-function $Q(\cdot,\cdot)$ is an optimal Q-function.
% \end{corollary}

\paragraph{Terminal Rewards.} At this point, one may wonder how we should assign a reward $r(s_a)$ upon the arrival at state $s_a$. To encourage the agent finds $\mc S_{T}$ while avoiding $\mc S_{T^-}$, a na\"ive reward assignment method is 
\begin{equation}
    r(s) = 
    \begin{cases}
        B & \text{if } s\in \mc S_{T}\\
        -B & \text{if } s\in \mc S_{T^-}\\
        0 &
        \text{otherwise}
    \end{cases},
\end{equation}
in words, the agent only receive a reward $(B>0)$ when it reaches the terminal states. This na\"ive reward design method is adopted in the training of AlphaGo \cite{silver2016mastering}, where the agent receives a reward of $+1,-1,0$ upon win, lose, and draw, respectively.

\subsection{Setting}
\paragraph{MDP. }
Consider an finite-horizon discounted MDP represented by a quintuple $\mc M = (\mc S,\mc A, P, r, \gamma)$, where $\mc S = \{1,2,\dots, |\mc S|\}$, $\mc A = \{1,2,\dots, |\mc A|\}$ are the state and action sets, respectively. $\gamma \in (0,1)$ is the discount factor, $r:\mc S \times \mc A \mapsto [0,B]$ is the reward function of each state-action pair $(s,a)$. Let $P:\mc S\times \mc A\mapsto \Delta(\mc S)$ be the probability transition kernel of the MDP, where $P(s_a|s,a)$ denote the probability of transiting from state $s$ to state $s_a$ when taking action $a$, and $\Delta(\mc S)$ denote the probability simplex over $\mc S$, we use $\mb P\in \bb R^{|\mc S||\mc A|\times |\mc S|}$ as the state-action transition matrix.

\cb{You define reward function as a function over each state-action pair, but in the value function definition r takes in 2 states and one action}

A deterministic policy is a mapping $\pi:\mc S\mapsto \mc A$ that maps a state to an action, and the value function $V^\pi:\mc \mapsto \bb R$ of a policy $\pi$ is defined by
\begin{equation}
    \forall s \in \mc S:\quad V^\pi(s)\doteq \bb E\left[ \sum_{t=0}^\infty\gamma^tr(s_t,a_t,s_{t+1})|s_0=s \right],
\end{equation}
where $r(s_t,a_t,s_{t+1})$ is the reward at time $t$ and $a_t=\pi(s_t)$ is the action taken at the $t^\text{th}$ state $s_t$. The trajectory is generated based on transition kernel ($s_{t+1}\sim P(\cdot|s_t,a_t)$). The corresponding action-value function (or Q-function) $Q^\pi:\mc S\times \mc A\mapsto \bb R$ of a policy $\pi$ is defined by 
\begin{equation}
    \forall (s,a) \in \mc S\times \mc A \quad Q^\pi(s,a) \doteq \bb E\left[\sum_{t=0}^\infty\gamma^t r(s_t,a_t,s_{t+1})|s_0 = s,a_0 = a\right],
\end{equation}
where the actions {\em after} the initial action $a_0$ follows policy $\pi$ (i.e., $a_t=\pi(s_t),\forall t\geq 1$.)

Let $\pi^\star$ denote the optimal policy that maximizes $V^\pi(s)$ and $Q^\pi(s,a)$, for all $s\in\mc S$ and $(s,a)\in \mc S\times \mc A$. 
Unlike many previous works \cite{wainwright2019variance,yang2019sample,sidford2018near,sidford2018variance,li2020breaking,agarwal2020model} that assume the reward $r(s,a)$ as a mapping from state-action pair to $\bb R$, our reward $r(s,a,s_a)$ also takes the next state $s_a$ into consideration. Because many RL applications \cite{silver2016mastering,silver2016mastering,pathak2017curiosity,dubeyICLRW18human,ye2020towards,liu2020learning} adopt sparse rewards, that is, the agent only receives reward when it reaches a subset of $\mc S$. \cb{Previous sentence is incomplete sentence}

\paragraph{Start states and terminal states.}
In order to build a better connection between the MDP model and the real world reinforcement learning, we let $\mc S_S, \mc S_T(|\mc S_S|,|\mc S_T|\ll|\mc S|)$ denote the set of start states and terminal states \cite{bertsekas2019reinforcement} of $\mc S$, respectively. That is, the whole reinforcement learning process starts from $s\in \mc S_S$ and stops once the agent reaches any state $s\in \mc S_T$ and one can understand $\mc S_{T}$ as the {\em winning states}.

\subsection{The Goal of Reinforcement Learning}

In theoretical RL, we often assume the rewards $r(s,a,s_a)$ already exist, and the goal of RL is to find a policy that produces a trajectory with the maximal total reward. However, from a practical perspective, the rewards are usually {\em unknown} and the goal of RL is to {\em design} a proper reward function $r(s,a,s_a)$ for the tuple $(s, a, s_a)$, so that the agent can ``easily'' learn a policy that finds the desirable terminal states $\mc S_{T}$ (preferably in the minimum time horizon).\footnote{Not only the reward function, sometimes the state set $\mc S$ and action set $\mc A$ are also well engineered.}

\paragraph{Theoretical RL.} Theoretical RL works usually consist of the following steps:
\begin{enumerate}
    \item Assume there exists an MDP $\mc M(\mc S,\mc A,P,r,\gamma)$ that contains state set $\mc S$, action set $\mc A$, transition matrix $P$, reward function $r$ and discount factor $\gamma$.
    \item Using empirical state-action pairs and the subsequent states $(s,a,s_a)$ to estimate the value function $V(s), \forall s\in \mc S$ or Q-function  $Q(s,a),\forall (s,a)\in \mc S\times \mc A$.
    \item Output a policy $\pi^\star$ that maximizes the overall (expected) discounted reward.
\end{enumerate} 

\paragraph{Practical RL.} In comparison, practical RL works usually have the following steps:
\begin{enumerate}
    \item Given a task, design the state set $\mc S$, action set $\mc A$, reward function $r$, discount factor $\gamma$.
    \item Calculate (most of the time approximate) the value function $V(s), \forall s\in \mc S$ or Q-function $Q(s,a),\forall (s,a)\in \mc S\times \mc A$.
    \item Output a policy $\pi^\star$ that maximizes the overall (expected) discounted reward.
    \item Check the performance of $\pi^\star$ on the given task, and redesign $\mc S,\mc A,r,\gamma$ and the approximation of $V(s),Q(s,a)$ for improvement. 
\end{enumerate} 

Although both theoretical RL and practical RL want to find a policy $\pi^\star$ that maximizes the overall discounted reward of an MDP,  the main difference between theoretical and practical RL is that, theoretical RL aims at solving a given MDP, while practical RL also attempts to correctly design the MDP such that a specific task is completed. In terms of evaluation, theoretical RL cares more about the sample complexity or computational complexity of solving MDP, while practical RL focuses on the performance of the task (i.e., performance against the best human player). 


\subsection{Motivation}
\subsubsection{Theoretical Optimality of Practical Reinforcement Learning}

As mentioned in the previous subsection, theoretical RL and practical RL have different goals. In order to bridge the gap between theoretical RL and practical RL, our first motivation is to {\em provide a theoretical framework that characterizes the optimality of practical RL (in terms of Q-function)}.

\subsubsection{Intermediate Rewards}
The other motivation of this work is to {\em study how different reward functions affect the RL training}, with the main focus on {\em intermediate rewards}, as opposed to the {\em sparse rewards}.

Both intermediate rewards and sparse rewards appear widely in practice. From a practical perspective, one may consider RL as a path finding problem: we want to find a policy that guides the agent to reach the terminal states $\mc S_{T}$. For that purpose, many practical works \cite{silver2016mastering,silver2017mastering,berner2019dota,vinyals2017starcraft,vinyals2019grandmaster,ye2020towards,schrittwieser2020mastering,liu2020learning} assign positive rewards to the agent on winning and negative rewards on losing. As for the rewards at the other states, a na\"ive design is to set them to 0 and only keep the rewards at terminal states, which is known as the {\em sparse rewards} setting.

However, as shown in \cite{pathak2017curiosity,berner2019dota}, RL tasks with sparse rewards are hard to train in general, as the agent need to explore the whole state-action space to discover the terminal states with the highest reward. In fact, based on the prior knowledge about the tasks, many practical works first identify some {\em intermediate states} $\mc S_{I}$, known as states which must have been visited by the agent before reaching $\mc S_{T}$, and assign intermediate rewards to the agent upon the agent's arrival at the intermediate states. 

One can view each intermediate state $s_i\in \mc S_I$ as a ``one way checkpoint'', namely, in one episode, after visiting an intermediate state $s_i$, the agent will not able to visit $s_i$ again. Consequently, in one episode, the intermediate rewards $r(s,a,s_i)$ can only be obtained once. The concept of intermediate states and intermediate rewards have been widely adopted in practice. For example, in Montezuma's Revenge \cite{Brockman2016OpenAI}, the agent needs to obtain a key before opening a door, but the key can only be obtained once. Another example is that, in the Dota2 game \cite{berner2019dota}, the agent earns rewards by unlocking Mega creeps\footnote{See Table 6 of \cite{berner2019dota}.} and the Mega creeps of the agent's team can only be unlocked once.\footnote{More information on the rules and gameplay of Dota are available online; i.e., \url{https://purgegamers.true.io/g/dota-2-guide/}.}

\subsubsection{Maze} \cb{Note that intermediate states here are not "one way checkpoints"}
\label{subsubsec:maze}
Suppose we want to solve the maze problem shown in \Cref{fig:maze} using reinforcement learning. A na\"ive setting is to consider each block in the maze as a state. The agent can take an action from $\{\text{left},\text{right},\text{up},\text{down}\}$. In this example, 
since the cyan path is the only solution to the maze, we may conclude that the states of the cyan path are in $\mc S_I$ and designate the states as follows:
\begin{itemize}
    \item $\mc S_S = \{\text{the blue circle}\}$
    \item $\mc S_{T} = \{\text{the green circle}\}$
    \item $\mc S_{I} =  \{\text{states on the cyan path}\}$
\end{itemize}


In terms of rewards, a na\"ive method adopts the sparse rewards setting where the agent only receives rewards once it arrives at the terminal states $\mc S_{T}$.
\begin{equation*}
        r(s,a,s_a) = \begin{cases}
        r(s,a,s_a) = B >0 & \text{when } s_a \in \mc S_{T},\forall (s,a)\in \mc S\times \mc A,\\
        0 & \text{otherwise},
        \end{cases}
\end{equation*}
where we use $B$ to denote the terminal reward. However, if we are given additional information about the maze (say an intermediate state $s_I\in\mc S_I$ as shown in \Cref{fig:maze}), we can assign an intermediate reward to the agent upon the agent's arrival at $s_I$:
\begin{equation}
    \label{eq:Int_Reward_Maze}
        r(s,a,s_a) = \begin{cases}
        r(s,a,s_a) = B >0 & \text{when } s_a \in \mc S_{T},\forall (s,a)\in \mc S\times \mc A,\\
        r(s,a,s_a) = B_I >0 & \text{when } s_a =s_I,\forall (s,a)\in \mc S\times \mc A,\\
        0 & \text{otherwise},
        \end{cases}
\end{equation}
where $B_I$ is the intermediate reward. We hope that such new rewards \eqref{eq:Int_Reward_Maze} would facilitate the original RL problem (in terms of either sample complexity of computational complexity). Even though it seems to be unnatural to introduce intermediate states in the middle of a maze, we hope this simple example conveys the idea of intermediate rewards. As will be seen in \Cref{subsubsec:pacman}, the intermediate rewards naturally fits into the Pacman Game setting.

\subsubsection{The Pacman Game}
\label{subsubsec:pacman}
As shown in \Cref{fig:Pacman}, the Pacman game consists of these following elements: the position of the Pacman (agent), the position of the ghost, and food (white dots). The Pacman wins the game if it consumes all the food without encountering the ghost. 

In this case, it is intuitive to assign a (one-time) intermediate reward to the Pacman once it consumes a food, as the agent can only consume a food once so it is unnecessary to revisit states with food. Again, we hope the intermediate reward facilitates the RL training on the Pacman game. 

\cb{Note that in this case, not all terminal states are winning (as stated in intro)}

\begin{remark}[Relation between Distance Function and Correct Actions]
Combining the reachability assumption (Assumption \ref{assump:reachability}) and Definition \ref{def:min_step_correct_step}, the distance function and the correct actions satisfy these following properties: 
\begin{itemize}
    \item Unlike conventional distance functions that are lower bounded by 0, the distance function \eqref{eq:def_distance} between two states $s,s^\prime\in \mc S$ satisfies $1\leq D(s,s^\prime)\leq \infty$, because the agent needs to take at least one action before moving to another state, and $D(s,s^\prime)= \infty$ if $s^\prime$ is not reachable from $s$. We shall also note that the distance between a state $s$ to itself could be infinity ($D(s,s)=\infty$), and such phenomenon happens when the state $s$ cannot be revisited.
    \item By assuming $\mc S_{T}$ is reachable from $s_0$, Assumption \ref{assump:reachability} directly implies that $D(s_0,\mc S_{T})<\infty$.
    \item Definition \ref{def:min_step_correct_step} implies that, $\forall s\in \mc S$ such that $D(s,\mc S_T)<\infty$, an incorrect action $a^-\in \mc A^-(s)$ will not move the state $s$ towards $\mc S_T$ ($D(s,\mc S_{T}) \leq D(s_{a^-},\mc S_{T})$), where $s_{a^-}$ is the subsequent state of state-action pair $(s,a^-)$.
    \item Assumption \ref{assump:reachability} (c) implicitly suggests that $\forall s\in reach_{\mc M}(s_0)\backslash\mc S_{T}$, $\mc A^+(s)\neq\emptyset$, because wrong actions will not move $s$ towards $\mc S_{T}$ and there always exists a path from $s$ to $\mc S_{T}$.
\end{itemize}
\end{remark}

==> response.tex <==
\newpage
\begin{center}
    {\bf Response to Reviewers}
\end{center}

\paragraph{Reviewer C:}

\begin{itemize}
    \item  This paper investigates the problem of intermediate reward design for reinforcement learning. The paper performs theoretical analysis of several conditions where intermediate rewards help an RL agent learn faster, and also performs some empirical studies to corroborate the theoretical results. The theory lines up well with intuitions that RL practioners have had for a long time and provides a nice framework for further studies into optimal reward design. Overall, I think this paper provides a valuable contribution to an important problem in RL (that of reward design) and will influence future research in the field. However, I think certain areas could be improved, namely the framing of the main messages and the empirical results.
    
    {\bf General Response to Reviewer C:} Thank you very much for your insightful comments and your appreciation in our work, we will try our best to address all your comments.
    \item Detailed Comments:
    \begin{enumerate}
        \item While I certainly appreciate that the paper is tackling the important problem of reward design, the word `hierarchical' in the title and other parts was a bit misleading to me. I immediately thought of connections to options, hierarchical policies, etc. but the meat of the paper is focused on reward design and how that affects value iteration. In fact, I think the notion of directed acyclic graphs (DAGs) might serve as a better analogy to think about the OWSP and OWMP results (ignoring the non-intermediate/non-terminal states which can have loops). I suggest the authors to reframe the writing to emphasize more on the intermediate reward design rather than hierarchical planning. I believe that this would ensure the results reach the right set of researchers working on ideas around reward design.
        
        {\bf Author Response:} Thanks for mentioning this part, after thorough consideration, we agree the contribution of this work focuses more on reward design rather than planning. Hence we have decided to change the title to ``Computational Benefits of Intermediate Rewards in Learning Goal-Reaching Policy Learning''. We have also largely updated the introduction and abstract to focus on comparing the intermediate states and terminal states as ``subgoals'' and ``goals'' in goal reaching tasks, and we believe the subgoals and goals better characterize our framework. 
        \item Proposition 4.1 seems like a straightforward observation from the convergence proofs for value iteration (Sutton and Barto, 1999). I'm not sure if this is a new result and could be moved to background (Section 3) instead of in Section 4. 
        
        {\bf Author Response:} Thank you for raising this point. Classical literature focuses on the convergence of value function $V_k(s) = V^\star(s)$ for all state $s\in \mc S$. Proposition 4.1 makes an important distinction: that the computational cost to identify a successful policy (which is arguably more important in practice) is far less than that required for the value function to converge. We need to keep Proposition 4.1, since understanding this phenomena for the sparse reward setting is elemental to understand the more complicated settings (OWSP and OWMP) in Section 4. To address your concern, we have added a paragraph (at the end of Section 4.1) to clarify the difference between proposition 4.1 and the proof of the convergence of synchronous value iteration via dynamic programming in classic literature. 
        
        \item All the results assume r(s, a) > 0. How would the findings change if this isn't the case (common in several domains when the agent performs a 'bad' action)? Some discussion on this would help.
        
        {\bf Author Response:} Thanks for mentioning this part. We have added one paragraph ({\bf Negative Rewards} in Section 7.2) that briefly discuss the potential effects of negative rewards. Rigorous studies of negative rewards indeed require extra investigations, and we would like to leave that to future.
        
        \item The experiments performed are all on small grid world environments, while the paper leads discussed domains like PacMan and Montezuma's revenge as examples where the OWSP and OWMP conditions hold. Why not demonstrate the effect of intermediate reward design on one of these environments as well? This would significantly help strengthen the paper and also make it more likely for empirical work on these domains to leverage the findings of this paper.
        
        {\bf Author Response:} Thank you again for raising this point. The main goal of our experiments is to justify our theoretical results: 1) adding intermediate rewards to one-way intermediate states reduce computational complexity; 2) there is a trade-off between computational complexity and the pursuit of the shortest path in the OWMP setting. We discussed some applications in Table \ref{tab:app_example} because some of these (Pacman, Montezuma, Dota2, StarCraft II, and Honor of Kings) tasks contain some ``salient'' states that cannot be revisited. But our theoretical results do not apply to these games due to other factors in these games (e.g., randomness, unequal magnitude of intermediate rewards, negative intermediate reward, etc.). Sorry for the confusion, we have added two paragraphs to clarify your concern. Please refer to
        \begin{itemize}
            \item the last paragraph in Section 3.2: ``Note that even though some of the practical tasks...''
            \item the second paragraph in Section 6: ``The main purpose of our experiments is to justify our theoretical results...''
        \end{itemize}
    \end{enumerate}
    \item Minor Comments:
    \begin{itemize}
        \item I suggest using different colors (maybe darker?) for the icons in the figures (Fig 1, etc.). They are not visible when the paper is printed in black and white.
        
        {\bf Author Response: }
        We have slightly darkened the icons in these Figures: Fig. 1, Fig. 3, Fig. 4, Fig. 5, and Fig. 6. We apologize that we cannot make the icons darker because the visibility of the numbers in the grids of Fig. 3, Fig. 4, Fig. 5, and Fig. 6 may be affected by darker icons. We also wish to keep the brightness level of all icons across Fig. 1, Fig. 3, Fig. 4, Fig. 5, and Fig. 6 to be the same from an aesthetic perspective, sorry for the inconvenience.
        
        \item Page 10: "large of enough" -> "large enough"
        
        {\bf Author Response:} Thanks for catching this typo, we have corrected it.
    \end{itemize} 
    
    Recommendation: Accept with minor revisions
\end{itemize}




\paragraph{Reviewer F:}
\begin{itemize}
    \item The paper studies computational benefits of adding intermediate rewards. In particular, they propose a theoretical investigation of adding intermediate rewards which is normally done in practice. The main takeaway is that adding intermediate rewards is generally helpful to speed up planning but if the rewards perturb the original MDP optimal policy then of course a planning algorithm can fail to find a near-optimal policy.

    \item Although the problem studied by the authors is novel---and well motivated in practice---the result are not very surprising and the paper does not require a sophisticated execution. While the article is well written, many claims, including the overall message, are not surprising.

    \item Overall I think this is fine as a first attempt, although the contribution seems to be a bit little for a journal like JAIR.
    
\end{itemize}
Recommendation: Accept

{\bf Author Response:} Thank you very much for your appreciation in our work!

\paragraph{Reviewer I:}

\begin{itemize}
    \item The paper focuses on cases where the intermediate states have hierarchical structures in the form of a required sequence of “special states” to be met in a certain order before reaching a terminal state. The paper presents theoretical results for a very limited class of MDPs, namely deterministic with sequence of irreversible intermediate states and only non-negative and equal rewards (equal rewards for terminal states and equal rewards for the intermediate states, but the two can be different). Also, all the theoretical results are limited to synchronous VI.
    
    
    {\bf Author Response: } Thanks for the comments. As mentioned by other reviewers, this is arguably the first work to study the reward designs under practically verifiable assumptions. At this point, we agree that the theoretical framework is limited, but it sets up a framework for future studies in reward design. To address your concern, we discuss the limitations and some future directions of this work in paragraph {\bf Negative Rewards, Unequal Magnitude Intermediate Rewards} in Section 7.2 and Section 7.3 Future Works.
    
    \item Although the formal results are somehow interesting, as presented, they only hold for a far too limited regime. Importantly, there is no clear way of extending the results to the stochastic case, nor is it clear how to handle cases with diverse intermediate rewards. This is in direct contrast to the authors claims of contributions.
    
    {\bf Author Response:} Thank you very much for this suggestion. In the updated introduction, we have 1) addressed the algorithm of interest is SVI; 2) clarified our contributions. Please refer to section 1.2. We have provided a section (Section 7.3) to discuss the future directions. We have added a paragraph to discuss the generalization to unequal magnitude intermediate rewards, please refer to {\bf Unequal Magnitude Intermediate Rewards} in Section 7.2.
    
    \item The presentation is also vastly redundant. Even for the current level of contribution, I would strongly suggest rewriting the paper altogether with a better and more thoughtful structure (I believe the paper can easily be shrunk to half in size).

    {\bf Author Response: } Thanks for mentioning the redundancy, we have removed/shorten some sections (see detailed in the later response) to improve the readability. We apologize for the redundancy, but we cannot shrink any sections/subsections of the current manuscript as it will affect the theoretical rigor.

    \item All in all, I don't see sufficient contribution for the JAIR's audience form the current submission without any major update. ONLY IF the above point can be addressed, I would encourage the authors to resubmit.
    
    {\bf Author Response:} Thank you again for the suggestions, we have largely updated the draft based on your comments.
    
    \item More detailed comments:
    \begin{itemize}
        \item Table 1 --> I found it (and the pacman example) quite confusing. There are important factors which are fully dismissed (learning rate and init values may play a key role on the impact of reward’s size). Line 4 is even more confusing (the dense-reward regime). Form the description it looks like that after the last pellet is eaten the game terminates, and I am guessing what the authors mean by “winning rates” is the percentage of times that pacman successfully eats the last pellet before being eaten by a ghost (is that right? Not clear from the text). If that is true, then the goal does not match the reward. Indeed, an optimal policy here will be "NOT to eat the last pellet" so that the game does not finish and pacman can accumulate even more per-step rewards. In other words, those game instances where pacman “wins” per se, are indeed game loss from the perspective of your reward signal. This is definitely NOT because of “incorporating too much prior knowledge” as stated in text (last paragraph of page 2).
        
        {\bf Author Response:} Thank you very much for addressing this point, we apologize for the confusion. 
        \begin{itemize}
            \item Yes, the winning condition of the Pacman in our experiments in Sec 1.1 is to ``consume all food before being caught by the ghost''. We have edited the second sentence in the second paragraph of Section 1.1 to clarify the winning condition: ``In the Pacman game, the agent (Pacman) wins when it consumes all the food before being caught by the ghost''.
            \item We agreed that ``incorporating too much prior knowledge'' is not appropriate enough to characterize the main message of Section 1.1, we have updated the original sentence to ``However, design rewards based on prior knowledge sometimes could negatively affect the performance.'' (please refer to the second last sentence in Section 1.1).
        \end{itemize}
        We shall also clarify that, the main message of this section is to provide some intuition of when adding intermediate rewards based on prior knowledge could be either benefit or harm accomplishing fthe tasks of interest, as adding intermediate rewards may affect the optimal policies. As you have suggested, since changing the reward functions may change the optimal policy, the main purpose of this work is to provide a first attempt to leverage the computational complexity (RL with sparse terminal rewards are generally computationally expensive e.g., see \cite{kakade2002approximately}) and the correctness of the optimal policies when adding intermediate rewards.
        \item The pacman experiment has a negative reward, yet your formal settings only allows for positive rewards.
        
        {\bf Author Response:} Thanks for mentioning this, we indeed added negative rewards in the Pacman experiments in Section 1.1. Please refer to the caption in Table 1. We did not include such details of terminal rewards (+10 for winning and -10 for losing) in the main text because we want to leave all details of reward design in Table \ref{tab:experiments-1g} for consistency. 
        \item The paragraph before definition 3.4: The authors say: “Assumption 3.3 indicates that from a given state s, only a few intermediate states can be directly visited (without first visiting any other intermediate states)”. Not sure I follow this, “a few” as compared to what? Also, there is no restriction on “n” in Assumption 3.3. I can easily make an example that “many” intermediate states (compared to the total number of states) can be directly visited; think of a grid world where the agent is at the middle surrounded by several rewarding states and the radius of the grid is small (hence there are not too many more states than the rewarding ones around the agent).
        
        {\bf Author Response: }Thanks for raising this point. The ``a few'' is comparing to all intermediate states. We apologize for the confusion, and we have edited the ``a few'' to ``not every''. Hope that improve the readability, please refer to the second last sentence before Definition 3.4: ``not every intermediate state $s_i\in\mc S_I$ can be directly visited (without first visiting any other intermediate states).''
             
        % \item \cb{I would remove this bullet point entirely. The first bullet point is sufficient to answer the reviewer's concern, and this second bullet point just raises more confusion. I don't think they were confused about 'one-way'} We have provided an example to clarify your confusion regarding Assumption \ref{assump:OneWayIntermediateStates} and Assumption \ref{assump:diff_settings_IS}. In Assumption \ref{assump:diff_settings_IS}, we are assuming that Assumption \ref{assump:OneWayIntermediateStates} holds. That is, all intermediate states are actually {\em one-way} (cannot be revisited). In the situation you are raising, suppose we provide some locations where the agent receives intermediate rewards upon its arrival (as shown in Figure 1). It is true that all locations where the agent receive intermediate rewards are directly reachable, but the locations themselves should not be consider as a state. Instead, when there are intermediate rewards that can only be obtained once in one episode (like Pacman), we believe a state should consist of 1) the location of the agent 2) the location of available intermediate rewards. So in the example shown in Figure 1, suppose we can start at any location, then even though the available locations is 9, but the total number of state should be $9\times(4+3+2+1) = 90$, where $9$ is the number of possible locations of the agent and $4+3+2+1$ is the number of possible locations of the remaining locations that grant one-way intermediate rewards. Therefore, if there is any one-way location that provide one-way intermediate rewards, the number of states is much bigger than the number of potential locations of the agent (as shown in Figure 1, even if the agent's position in $s_1,s_2$ are the same, but $s_1,s_2$ are considered as different states due to the different available rewards).
            
        %     \begin{figure}[ht]
        %         \centering
        %         \input{value_grid/author_response_ow}
        %     \end{figure}
        \item Theoretical results of section 4 are completely limited to synchronous VI (and of course only for deterministic dynamics), while the claims of contributions at the beginning of the paper sound rather generic.
        
        {\bf Author Response: }Thanks for the suggestion, we apologize for the confusion. We have updated the contribution part in Section 1 introduction. Please refer to the last paragraph (Our Contributions) of Section 1.2.
    \end{itemize}
    \item Minors:
    \begin{itemize}
        \item Second line before definition 2.1: … set of terminal state $\mathcal{S}_T$ ...
        
        {\bf Author Response: }Thanks for catching this grammar error, we have updated it accordingly.
        \item Would be more clear to explicitly say it forefront that you consider deterministic, episodic MDP, as you assume deterministic transitions and that from each state there exist a path to a terminal state. Also, if that’s the case, the sequence of actions from init state to a terminal state might be defined as finite.
        
        {\bf Author Response: }Thanks for the suggestion, we have updated the introduction on the settings.
        \item There are numerous unnecessary introductory paragraphs before each part stating that what is going to be presented in the coming section/subsection. These are all redundant and make the reader annoyed. A far better practice is to be concise and precise [but not too concise]. I would suggest removing all such parts.
        
        {\bf Author Response: } Thank you very much for this suggestion and sorry for the redundancy, we have updated the following introductory parts:
        \begin{itemize}
            \item we have shortened the introductory paragraph of Section 2.2
            \item we have removed the introductory paragraph of Section 3
            \item we have shortened the introductory paragraph of Section 3.2
            \item we have shortened the introductory paragraph of Section 4.2
            \item we have shortened the introductory paragraph of Section 4.3
            \item we have shortened the introductory paragraph of Section 4.4
            \item we have shortened the introductory paragraph of Section 5
        \end{itemize}
        \item Page 9, the first full line bellow table 2: typo (visit).
        
        \item Page 10, second last paragraph: large enough (remove of).
        
        {\bf Author Response:} Thanks for catching the two typos, we have fixed them.
    \end{itemize}
    Recommendation: Reject with encouragement to resubmit
\end{itemize}


\paragraph{Reviewer J:}
\begin{itemize}
    \item This paper provides a theoretical justification for the use of intermediate rewards to speed up convergence in reinforcement learning. In particular, the authors consider several forms of MDPs and develop upper bounds on the number of iterations necessary to achieve a solution of the greedy policy within a policy iteration approach. The authors prove that while the number of iterations in the absence of intermediate rewards (a.k.a. sparse reward setting) is upper bounded by the distance between the initial and target states, with intermediate rewards the number of iterations is roughly proportional to the distance between consecutive intermediate rewards, which can be much shorter.
    \item Although the tools used in this work, as well as the final outcomes, are quite intuitive, I appreciate that the authors have made this effort, and I hope that it would lead to a better understanding of the success and limitations of existing RL approaches. Thus, I feel that this work makes a good contribution to the community.
    \item The paper overall is quite accessible, and I don't have particular criticism besides suggestions on improving the readability, organization and presentation, on which I elaborate below.
    
    {\bf General Response to Reviewer J:} Thank you very much for your appreciation in our work and you comments, we will try our best to improve our draft based based on your suggestions.
    \item Additional remarks: In general, the text would benefit from higher precision and rigor. Currently, many statements are overly handwavy. Consider for instance the following comments and suggestions: 
    \begin{itemize}
        \item The term "computational benefit", which is used extensively in the abstract and the intro, is formally defined in Section 4. It would be beneficial to be more concrete already in the introductory text and abstract, by providing an informal description of the main results in Section 4. 
        
        \item Please be more explicit about the term intermediate and sparse reward in the abstract and intro.
        
        {\bf Author Response:} Thank you very much on addressing the two points above, we have updated our abstract and introduction accordingly.
        \item Section 1.1: be more precise when stating tat the configuration of the maze problem remains unchanged. I.e., as you move from one state to another the configuration is changing by definition.
        
        {\bf Author Response:} Thanks for mentioning this point, we have edited the first paragraph of section 1.1. Please see the second sentence: ``For the Maze problem, if we assume one episode ends if and only if the agent reaches the goal, then the Maze problem does not have a hierarchical structure, since all previously visited states can be revisited in one episode.''
        \item Citations needed to the claim on page 3 that "Many practical RL tasks implictly adopt this one-way property". 
        
        {\bf Author Response:} Thank you for the comment, we have added some related references.
        \item Figure 4: It would be worth summarizing the implications of this figure.
        
        {\bf Author Response:} Thanks again for the suggestion, we have added one sentence in the paragraph {\bf The OWSP Setting} ``Intuitively, Figure 4 suggests that the computational complexity of finding a policy that reaches the terminal states can be reduced by rewarding the one-way intermediate states.'' which briefly summarize the intuition of Figure 4 right after its introduction.
        \item Statement of contribution should be more precise. To get the main idea the reader is forced to read all the way through section 4.
        
        
        {\bf Author Response: } Thanks for the suggestion, the introduction has been largely updated. We have updated section 1.2 and provide more details of 1) the one-way intermediate states; 2) the sparse reward setting and the intermediate reward settings; 3) our contributions. Please see the updated section 1.2.2. 
        \item Provide citation for the statement that "Assumption 3.2" is widely adopted.
        
        {\bf Author Response: } Thanks again for the comment, we have added related citations and related this part to the discussion in Section 3.2.
        \item When stating the assumptions in Section 3.1, explain why they are important or necessary in your analysis.
        
        {\bf Author Response:} Thank you very much for addressing this issue, we have added one paragraph in Section 3.1 (the last paragraph of Section 3.1) to discuss the connection between the assumptions to our main result: ``The aforementioned assumptions (Assumption \ref{assump:OneWayIntermediateStates}, \ref{assump:diff_settings_IS}, and \ref{assump:min_dist_IS}) are connected to our main results in the following respects...''
        \item It would be worth going into a bit more detail in explaining how Pacman satisfies Assumption 3.3(b), by, e.g., providing a description of its MDP. 
        
        {\bf Author Response:} Thank you very much for highlighting this, we have edited the second paragraph in section \ref{subsec:InterpretInterState}, please refer to the updated discussion of the pacman game at these following sentences: ``If we consider each state in the Pacman game consists of... Hence each episode of the Pacman game contains $n$ (the total number of food) intermediate states, and these states appear in the order in which the number of available food is decreasing.''
        \item Most of Section 3.2 focuses on assumption 3.3, and it's unclear how the other assumption come into play.
        
        {\bf Author Response: } Thanks for the comment. We have added one paragraph at the end of Section 3.1 to discuss why we plan Section 3.2 to only discuss Assumption 3.3. Please refer to the paragraph: ``The aforementioned assumptions (Assumption \ref{assump:OneWayIntermediateStates}, \ref{assump:diff_settings_IS}, and \ref{assump:min_dist_IS}) are connected to our main results in the following respects...'' 
        
        We shall also clarify that, Assumption \ref{assump:diff_settings_IS} is based on Assumption \ref{assump:OneWayIntermediateStates}, so Section 3.2 is discussing Assumption \ref{assump:diff_settings_IS} and \ref{assump:OneWayIntermediateStates} together. As for Assumption \ref{assump:min_dist_IS}, we consider it less important because it does not characterize the ``connection'' of the MDP graph, and it is only used for quantitative purpose in the proof. Hence, we only focusing on discussing the practicality of Assumption \ref{assump:diff_settings_IS} and \ref{assump:OneWayIntermediateStates} in Section 3.2, because they are task dependent.
        \item Sec 3.3: State what $B$ and $B_I$ mean. 
        
        {\bf Author Response:} Thank you again for the suggestion. We have added one sentence (the first sentence of the second paragraph in Section 3.3) that explains $B$ and $B_I$: ``In Table \ref{tab:reward_setting}, we assume the agent receive terminal rewards $B$ once it reaches $s_t\in \mc S_T$, and receive intermediate rewards $B_I$ once it reaches an intermediate state $s_i\in \mc S_I$. ''
        
        \item Sec 4.3: Give intuition how the proof of Prop 4.2 breaks when applied to OWMP. 
        
        {\bf Author Response:} Thanks for the suggestion, we have added one sentence at the end of the first paragraph in Section 4.3, please see: ``From a theoretical perspective, Proposition \ref{prop:com_comp_inter_reward} for the OWSP setting cannot be directly generalized to the OWMP case...'' 
        \item Proof sketches are overly vague. Please provide more details about the proofs and the techniques used therein.
        
        {\bf Author Response:} Thanks for the suggestion, we have updated two paragraphs (the paragraph below Theorem \ref{thm:find_closest_IS} and Theorem \ref{thm:find_closest_TerminalState}) and provided more details to the sketch proof.
        
        \item Sec 6: it would be worth comparing the theoretical bounds with the practical results, to get an understanding about how tight the bounds are. 
        
        {\bf Author Response:} Thanks for raising this point. Unfortunately our result in Theorem \ref{thm:find_closest_IS} and Theorem \ref{thm:find_closest_TerminalState} only provide {\em sufficient} conditions, so we cannot say more regarding how tight the bounds are. In addition, it is hard to provide necessary conditions for Theorem \ref{thm:find_closest_IS} and Theorem \ref{thm:find_closest_TerminalState} {\em without} making extra assumptions on the MDP. We sincerely apologize for the confusion, as the tightness of such bound is not the main contribution of this work. We believe studying the tightness of the bound is important, and we would like to leave that to future (see section 7.3 ``future work'').
        \item The paper lacks a discussion of future work. E.g., do you believe that your result can be extended beyond the OWMP setting? What are the main limitations of your analysis?
        
        {\bf Author Response:} Thanks for the suggestion, we have added an section to discuss future works (section 7.3 future works).
    \end{itemize}
    \item Comment of equal magnitude of intermediate rewards:
    
    At the end of Sec 3 it is claimed that the analysis can be generalized beyond equal magnitude of intermediate rewards (EMIR). If you believe that this is the case please elaborate. Let me mention that it might be possible to convert settings with unequal intermediate rewards to EMIR by splitting or batching rewards, so that the new problem is equivalent to the original one (albeit with possibly longer paths between intermediate rewards).
    
    {\bf Author Response:} Thanks for bringing this up, we have added one paragraph in the discussion section (Sec. 7.2) to discuss the unequal magnitude of intermediate rewards. We believe that generalizing the equal magnitude intermediate rewards to unequal magnitude requires some extra assumptions on the scaling of different intermediate rewards, but the key techniques are the same as the equal magnitude case. Please refer to the paragraph ``Unequal Magnitude Intermediate Rewards'' in Section 7.2.
    \item Typos:
    \begin{itemize}
        \item p9: "vis it"
        \item p10 "large {\em remove}\{of\} enough"; "discuss {\em replace\{these\} with \{the\} } following"; NOW hasn't been defined yet.
        \item p22: "at at"
    \end{itemize}
    {\bf Author Response:} Thanks for checking the typos and mentioning the NOW setting, we have 1) updated all typos; 2) edited the paragraph right below Table 4 to introduce the NOW setting and related the OWSP, OWMP, and NOW to their required assumptions in Table 4.
    
    Recommendation: Accept with minor revisions
\end{itemize}
\newpage

==> table/nips_app_example.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table for NIPS submission %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{wraptable}{r}{50mm}
    \vspace{-1.2em}
    \centering
    \footnotesize
    \begin{tabular}{lcc}
        \toprule
        Assumption \ref{assump:diff_settings_IS} & (a) & (b)\\
         \midrule
         Pacman (\cite{racaniere2017imagination})& \xmark & \cmark \\
         Montezuma (\cite{Brockman2016OpenAI})& \cmark &  \cmark \\
        %  MiniGrid (\cite{gym_minigrid})& \cmark & \cmark \\
         Go (\cite{silver2016mastering,silver2017mastering})& \xmark & \xmark \\
         Dota2 (\cite{berner2019dota}) & \xmark & \cmark\\
         StarCraft II (\cite{vinyals2017starcraft,vinyals2019grandmaster})& \xmark &  \cmark \\
         Honor of Kings (\cite{ye2020towards})& \xmark & \cmark \\
        \bottomrule
    \end{tabular}
    \vspace{-0.5em}
    \caption{\footnotesize Examples of some RL applications that adopt different settings in Assumption \ref{assump:diff_settings_IS}.}
    \label{tab:app_example}
    \vspace{-1.8em}
\end{wraptable}

==> table/nips_experiment.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    \begin{tabular}{rcc|rcc}
        \toprule 
        \multicolumn{3}{c|}{Maze (Figure \ref{fig:sparsemaze} and \ref{fig:intermaze})} & \multicolumn{3}{c}{3-Door (Figure \ref{fig:3door})}\\
        \toprule
        \# Episodes & Sparse & Intermediate & \# Episodes & Sparse & Intermediate\\
        \midrule 18	& 6/100 &59/100 & 40 &	3/100 & 90/100 \\
        \midrule 24	& 7/100 &82/100 & 80 & 10/100 & 100/100 \\
        \midrule 30	& 6/100 &95/100 & 120 &	43/100 & 100/100\\
        \midrule 36	& 10/100 &  100/100 & 160 & 74/100& 100/100\\
        \bottomrule
    \end{tabular}
    \caption{\footnotesize Asynchronous Q-learning: Computational Complexity. We report the number of wins out of 100 trials (100 training sessions evaluated once each) after different training episodes for both the sparse reward and intermediate reward settings.}
    \vspace{-1em}
    \label{tab:minigrid1}
\end{table}

\begin{table}[ht]
    \centering
    \footnotesize
    \begin{tabular}{rcccccc}
        \toprule
        \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Setting 1: +10} & \multicolumn{3}{c}{Setting 2: +1000}\\
        \midrule
        \# Episodes & Wins & Rewards & Steps & Wins & Rewards & Steps\\
        \toprule 50 & 64/100& 11.28 $\pm$ 2.08 & 95.52 $\pm$ 82.58  & 71/100 & 11.12 $\pm$ 2.30 & 84.39 $\pm$ 79.48\\
        \midrule 150 & 99/100 & 11.2 $\pm$ 2.03 & 24.71 $\pm$ 18.10 & 100/100 & 11.06 $\pm$ 1.99 & 22.53 $\pm$ 3.56 \\
        \midrule 350 & 100/100 & 11.1 $\pm$ 1.93 &  22.65 $\pm$ 3.40 & 100/100 & 10.14 $\pm$ 2.60 &  20.88 $\pm$ 4.70 \\
        \midrule 750 & 100/100 & 11.18 $\pm$ 1.80 & 22.85 $\pm$ 3.24 & 100/100 & 9.24 $\pm$ 2.85 & 19.39 $\pm$ 5.54 \\
        \midrule 1550 & 100/100 & 11.64 $\pm$ 1.42 & 23.36 $\pm$ 2.62  & 100/100 & 5.52 $\pm$ 1.10&  12.95 $\pm$ 1.64\\
        \midrule 3150 & 100/100 & 12.0 $\pm$ 0.0 & 24.0 $\pm$ 0.0 & 100/100 & 4.46 $\pm$ 0.84 &  12.23 $\pm$ 0.42 \\
        \bottomrule
    \end{tabular}
    \caption{\footnotesize 4-Door (Figure \ref{fig:4door}) Trade-Off for Asynchronous Q-Learning. We report the number of wins out of 100 trials (100 training sessions evaluated once each), averaged total intermediate rewards, and averaged number of steps taken after different training episodes. The agent receives a terminal reward of +10 in Setting 1 +1000 in Setting 2. The agent also receives +2 for picking up a key and +2 for opening a door in both settings. The episode maxes out at 324 steps.} \vspace{-1em}\vspace{-1em}\vspace{-1em}
    \label{tab:minigrid3}
\end{table}


==> table/pre_work.tex <==
\begin{table}[H]
    \centering
    \small
    \begin{tabular}{lcccc}
        \toprule
        \multicolumn{1}{c}{Algorithm} & \multicolumn{1}{c}{Sample size range} & \multicolumn{1}{c}{Sample complexity} &\multicolumn{1}{c}{$\eps$-range}\\
        \toprule
        Phase Q-learning \cite{kearns1999finite} & $\left[\frac{|\mc S||\mc A|}{(1-\gamma)^5},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^7\eps^2}$ & $\left(0,\frac{1}{1-\gamma}\right]$\\
        \midrule
        Empirical QVI \cite{azar2013minimax} & $\left[\frac{|\mc S|^2|\mc A|}{(1-\gamma)^2},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^3\eps^2}$ & $\left(0,\frac{1}{\sqrt{(1-\gamma)|\mc S|}}\right]$
        \\
        \midrule Sublinear randomized value iteration \cite{sidford2018variance} & $\left[\frac{|\mc S||\mc A|}{(1-\gamma)^2},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^4\eps^2}$ & $\left(0,\frac{1}{1-\gamma}\right]$ \\
        \midrule
        Variance-reduced QVI \cite{sidford2018near} & $\left[\frac{|\mc S||\mc A|}{(1-\gamma)^3},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^3\eps^2}$ & $\left(0,1\right]$\\
        
        \midrule Randomized primal-dual method \cite{wang2020randomized}  & $\left[\frac{|\mc S||\mc A|}{(1-\gamma)^2},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^4\eps^2}$ & $\left(0,\frac{1}{1-\gamma}\right]$ \\
        \midrule Empirical MDP + planning \cite{agarwal2020model} & $\left[\frac{|\mc S||\mc A|}{(1-\gamma)^2},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^3\eps^2}$ & $\left(0,\frac{1}{\sqrt{1-\gamma}}\right]$ \\
        \midrule Perturbed empirical MDP + planning \cite{li2020breaking} & $\left[\frac{|\mc S||\mc A|}{1-\gamma},\infty\right)$ & $\frac{|\mc S||\mc A|}{(1-\gamma)^3\eps^2}$ & $\left(0,\frac{1}{1-\gamma}\right]$ \\
        \bottomrule
    \end{tabular}
    \caption{Algorithm and sample complexity of previous work in achieving $\eps$-error Q-function and value function.}
    \label{tab:previous_work}
\end{table}

% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.35\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0cm 0cm 1.5cm 1.5cm},clip]{fig/LossCurve_AngDiff/loss_plot.png}
%         \caption{Losses}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.35\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0cm 0cm 1.5cm 1.5cm},clip]{fig/LossCurve_AngDiff/AngDiff.png}
%         \caption{Angular Differences}
%     \end{subfigure}
%     \caption{Loss curves (a) and angular difference curves (b) during \num{300} training epochs of a NSGAN on the CelebA dataset. The clear jumps of the angular difference curves in (b) correspond to a qualitative transition of the NSGAN network as we will discuss later.}
%     \label{fig:Loss_AngDiff}
% \end{figure}

==> table/strategy.tex <==
\begin{table}[ht]
    \centering
    \small
    \begin{tabularx}{0.9\textwidth}{XcXX}
        \toprule
        \multicolumn{1}{c}{Assumptions} &
        \multicolumn{1}{c}{Suggestions} &\multicolumn{1}{c}{Strategies} & \multicolumn{1}{c}{Praticality} \\
        \toprule $\mc S_O$ is known & 1,2,4 & Assign arbitrary large one time reward $r_o(s^\prime, s, a)$ or recursive reward $r_r(s^\prime,s,a)<M(1-\gamma)$ to all states $s^\prime \in \mc S_O$. & This assumption is too strong for practice. We cannot directly infer $\mc S_N$ from many practical RL problems.\\
        \midrule part of $\mc S_N$ (or $\mc S_I$) is known & 1,2 & For $s^\prime \in \mc S_N$, we can assign arbitrary large one time reward $r_o(s^\prime, s, a)$ or recursive reward $r_r(s^\prime,s,a)<M(1-\gamma)$. For $s^\prime \in \mc S_I$, we can assign very small recursive reward $r_r(s^\prime,s,a)\ll M(1-\gamma)$ / small one time reward $r_o(s^\prime, s, a)$ that encourage the exploration. & This assumption is relatively practical, since we can directly infer the necessary states based on our prior knowledge of the RL problems.\\
        \midrule Nothing is known & None & This is the typical sparse reward RL setting & This assumption is slightly weak for practice, as the agent is given no extra information about the environment, it takes many computation resource to explore all possible state-action pairs.\\
        \bottomrule
    \end{tabularx}
    \caption{Strategies of reward designing (under different assumptions) in solving the maze MDP in Figure \ref{fig:maze_c}. These assumptions are sorted from their practicality.}
    \label{tab:strategy}
\end{table}

% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[t]{0.35\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0cm 0cm 1.5cm 1.5cm},clip]{fig/LossCurve_AngDiff/loss_plot.png}
%         \caption{Losses}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.35\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0cm 0cm 1.5cm 1.5cm},clip]{fig/LossCurve_AngDiff/AngDiff.png}
%         \caption{Angular Differences}
%     \end{subfigure}
%     \caption{Loss curves (a) and angular difference curves (b) during \num{300} training epochs of a NSGAN on the CelebA dataset. The clear jumps of the angular difference curves in (b) correspond to a qualitative transition of the NSGAN network as we will discuss later.}
%     \label{fig:Loss_AngDiff}
% \end{figure}
